Fairness Scheduling for Coded Caching in Multi-AP Wireless Local Area Networks

Coded caching (CC) exploits cumulative cache memory at user devices and coding to transform unicast traffic into multicast transmissions. While information theoretic results show significant gains over uncoded caching for various network topologies, its practical benefits remain unclear. In this work, we investigate CC for on-demand video streaming over large wireless local area networks, where multiple users are served simultaneously by spatially distributed access points. Users asynchronously request video chunks from a content library. We propose a decentralized, asynchronous, and location-independent cache placement scheme combined with an "over IP" delivery mechanism operating at higher network layers, leaving the physical and MAC layers unchanged. For this scheme, we characterize the achievable goodput region, where goodput is defined as the number of video chunks per unit time delivered to users' playback buffers, and formulate the corresponding fairness problem as a convex maximization. We develop a dynamic scheduling algorithm that provably achieves the optimal fairness point under stationary conditions with reduced complexity, and introduce a heuristic to further lower complexity. Numerical results demonstrate significant gains over baseline schemes, including conventional prefix caching, orthogonal sub-channel allocation with spatial reuse, and a CSMA-inspired distributed coordination approach, showing that CC can be implemented as a scalable and compatible over IP solution for existing WLANs.

==> Figs/New_dynamic_TWC.tex <==
U1 U2 U3 U4 U5 U6 U7 Slots
1.50000000000000	0	0	1	0	1	0	1
0.750000000000000	0	0.500000000000000	1	0.500000000000000	0.500000000000000	0	2
1	0	0.333333333333333	1	0.333333333333333	0.666666666666667	0	3
0.750000000000000	0	0.500000000000000	1	0.500000000000000	0.500000000000000	0	4
0.900000000000000	0	0.400000000000000	1	0.400000000000000	0.600000000000000	0	5
1	0	0.333333333333333	1	0.500000000000000	0.500000000000000	0	6
0.857142857142857	0	0.428571428571429	1	0.428571428571429	0.571428571428571	0	7
0.937500000000000	0	0.375000000000000	1	0.500000000000000	0.500000000000000	0	8
0.833333333333333	0	0.444444444444444	1	0.444444444444444	0.555555555555556	0	9
0.900000000000000	0	0.400000000000000	1	0.500000000000000	0.500000000000000	0	10
0.818181818181818	0	0.454545454545455	1	0.454545454545455	0.545454545454545	0	11
0.875000000000000	0	0.416666666666667	1	0.500000000000000	0.500000000000000	0	12
0.923076923076923	0	0.384615384615385	1	0.461538461538462	0.538461538461538	0	13
0.857142857142857	0	0.428571428571429	1	0.500000000000000	0.500000000000000	0	14
0.900000000000000	0	0.400000000000000	1	0.466666666666667	0.533333333333333	0	15
0.843750000000000	0	0.437500000000000	1	0.500000000000000	0.500000000000000	0	16
0.882352941176471	0	0.411764705882353	1	0.470588235294118	0.529411764705882	0	17
0.833333333333333	0	0.444444444444444	1	0.500000000000000	0.500000000000000	0	18
0.868421052631579	0	0.421052631578947	1	0.473684210526316	0.526315789473684	0	19
0.825000000000000	0	0.450000000000000	1	0.500000000000000	0.500000000000000	0	20
0.857142857142857	0	0.428571428571429	1	0.476190476190476	0.523809523809524	0	21
0.818181818181818	0	0.454545454545455	1	0.500000000000000	0.500000000000000	0	22
0.847826086956522	0	0.434782608695652	1	0.478260869565217	0.521739130434783	0	23
0.812500000000000	0	0.458333333333333	1	0.500000000000000	0.500000000000000	0	24
0.840000000000000	0	0.440000000000000	1	0.480000000000000	0.520000000000000	0	25
0.807692307692308	0.0576923076923077	0.423076923076923	0.961538461538462	0.461538461538462	0.500000000000000	0	26
0.833333333333333	0.0555555555555556	0.407407407407407	0.962962962962963	0.481481481481481	0.481481481481481	0	27
0.803571428571429	0.0535714285714286	0.428571428571429	0.964285714285714	0.464285714285714	0.500000000000000	0	28
0.827586206896552	0.0517241379310345	0.413793103448276	0.965517241379310	0.482758620689655	0.482758620689655	0	29
0.800000000000000	0.0500000000000000	0.433333333333333	0.966666666666667	0.466666666666667	0.500000000000000	0	30
0.822580645161290	0.0483870967741936	0.419354838709677	0.967741935483871	0.483870967741936	0.483870967741936	0	31
0.796875000000000	0.0468750000000000	0.437500000000000	0.968750000000000	0.468750000000000	0.500000000000000	0	32
0.818181818181818	0.0454545454545455	0.424242424242424	0.969696969696970	0.484848484848485	0.484848484848485	0	33
0.794117647058824	0.0882352941176471	0.411764705882353	0.941176470588235	0.470588235294118	0.470588235294118	0	34
0.771428571428572	0.0857142857142857	0.428571428571429	0.942857142857143	0.457142857142857	0.485714285714286	0	35
0.791666666666667	0.0833333333333333	0.416666666666667	0.944444444444444	0.472222222222222	0.472222222222222	0	36
0.770270270270270	0.0810810810810811	0.432432432432432	0.945945945945946	0.459459459459460	0.486486486486487	0	37
0.789473684210526	0.0789473684210526	0.421052631578947	0.947368421052632	0.473684210526316	0.473684210526316	0	38
0.769230769230769	0.0769230769230769	0.435897435897436	0.948717948717949	0.461538461538462	0.487179487179487	0	39
0.787500000000000	0.0750000000000000	0.425000000000000	0.950000000000000	0.475000000000000	0.475000000000000	0	40
0.768292682926829	0.0731707317073171	0.439024390243902	0.951219512195122	0.463414634146342	0.487804878048781	0	41
0.750000000000000	0.107142857142857	0.428571428571429	0.928571428571429	0.452380952380952	0.476190476190476	0	42
0.767441860465116	0.104651162790698	0.418604651162791	0.930232558139535	0.465116279069767	0.465116279069767	0	43
0.750000000000000	0.102272727272727	0.431818181818182	0.931818181818182	0.454545454545455	0.477272727272727	0	44
0.766666666666667	0.100000000000000	0.422222222222222	0.933333333333333	0.466666666666667	0.466666666666667	0	45
0.750000000000000	0.0978260869565217	0.434782608695652	0.934782608695652	0.456521739130435	0.478260869565217	0	46
0.765957446808511	0.0957446808510638	0.425531914893617	0.936170212765958	0.468085106382979	0.468085106382979	0	47
0.750000000000000	0.125000000000000	0.416666666666667	0.916666666666667	0.458333333333333	0.458333333333333	0	48
0.734693877551020	0.122448979591837	0.428571428571429	0.918367346938776	0.448979591836735	0.469387755102041	0	49
0.750000000000000	0.120000000000000	0.420000000000000	0.920000000000000	0.460000000000000	0.460000000000000	0	50
0.735294117647059	0.117647058823529	0.431372549019608	0.921568627450980	0.450980392156863	0.470588235294118	0	51
0.750000000000000	0.115384615384615	0.423076923076923	0.923076923076923	0.461538461538462	0.461538461538462	0	52
0.735849056603774	0.113207547169811	0.433962264150943	0.924528301886793	0.452830188679245	0.471698113207547	0	53
0.750000000000000	0.111111111111111	0.425925925925926	0.925925925925926	0.462962962962963	0.462962962962963	0	54
0.736363636363636	0.136363636363636	0.418181818181818	0.909090909090909	0.454545454545455	0.454545454545455	0	55
0.723214285714286	0.133928571428571	0.428571428571429	0.910714285714286	0.446428571428571	0.464285714285714	0	56
0.736842105263158	0.131578947368421	0.421052631578947	0.912280701754386	0.456140350877193	0.456140350877193	0	57
0.724137931034483	0.129310344827586	0.431034482758621	0.913793103448276	0.448275862068966	0.465517241379310	0	58
0.737288135593220	0.127118644067797	0.423728813559322	0.915254237288136	0.457627118644068	0.457627118644068	0	59
0.725000000000000	0.125000000000000	0.433333333333333	0.916666666666667	0.450000000000000	0.466666666666667	0	60
0.737704918032787	0.122950819672131	0.426229508196721	0.901639344262295	0.467213114754098	0.459016393442623	0	61
0.725806451612903	0.120967741935484	0.435483870967742	0.903225806451613	0.459677419354839	0.467741935483871	0	62
0.714285714285714	0.142857142857143	0.428571428571429	0.888888888888889	0.452380952380952	0.460317460317460	0	63
0.726562500000000	0.140625000000000	0.421875000000000	0.890625000000000	0.460937500000000	0.453125000000000	0	64
0.715384615384615	0.138461538461539	0.430769230769231	0.892307692307692	0.453846153846154	0.461538461538462	0	65
0.727272727272727	0.136363636363636	0.424242424242424	0.893939393939394	0.462121212121212	0.454545454545455	0	66
0.716417910447761	0.134328358208955	0.432835820895522	0.895522388059702	0.455223880597015	0.462686567164179	0	67
0.727941176470588	0.132352941176471	0.426470588235294	0.897058823529412	0.463235294117647	0.455882352941176	0	68
0.717391304347826	0.152173913043478	0.420289855072464	0.884057971014493	0.456521739130435	0.449275362318841	0	69
0.707142857142857	0.150000000000000	0.428571428571429	0.885714285714286	0.450000000000000	0.457142857142857	0	70
0.718309859154930	0.147887323943662	0.422535211267606	0.887323943661972	0.457746478873239	0.450704225352113	0	71
0.708333333333333	0.145833333333333	0.430555555555556	0.888888888888889	0.451388888888889	0.458333333333333	0	72
0.719178082191781	0.143835616438356	0.424657534246575	0.890410958904110	0.458904109589041	0.452054794520548	0	73
0.709459459459459	0.141891891891892	0.432432432432432	0.891891891891892	0.452702702702703	0.459459459459460	0	74
0.700000000000000	0.160000000000000	0.426666666666667	0.880000000000000	0.446666666666667	0.453333333333333	0	75
0.710526315789474	0.157894736842105	0.421052631578947	0.881578947368421	0.453947368421053	0.447368421052632	0	76
0.701298701298701	0.155844155844156	0.428571428571429	0.883116883116883	0.448051948051948	0.454545454545455	0	77
0.711538461538462	0.153846153846154	0.423076923076923	0.884615384615385	0.455128205128205	0.448717948717949	0	78
0.702531645569620	0.151898734177215	0.430379746835443	0.886075949367089	0.449367088607595	0.455696202531646	0	79
0.712500000000000	0.150000000000000	0.425000000000000	0.887500000000000	0.456250000000000	0.450000000000000	0	80
0.703703703703704	0.166666666666667	0.419753086419753	0.876543209876543	0.450617283950617	0.444444444444444	0	81
0.695121951219512	0.164634146341463	0.426829268292683	0.878048780487805	0.445121951219512	0.451219512195122	0	82
0.704819277108434	0.162650602409639	0.421686746987952	0.879518072289157	0.451807228915663	0.445783132530121	0	83
0.696428571428571	0.160714285714286	0.428571428571429	0.880952380952381	0.446428571428571	0.452380952380952	0	84
0.705882352941177	0.158823529411765	0.423529411764706	0.882352941176471	0.452941176470588	0.447058823529412	0	85
0.697674418604651	0.156976744186047	0.430232558139535	0.883720930232558	0.447674418604651	0.453488372093023	0	86
0.689655172413793	0.172413793103448	0.425287356321839	0.873563218390805	0.442528735632184	0.448275862068966	0	87
0.698863636363637	0.170454545454545	0.420454545454545	0.875000000000000	0.448863636363636	0.443181818181818	0	88
0.691011235955056	0.168539325842697	0.426966292134831	0.876404494382023	0.443820224719101	0.449438202247191	0	89
0.700000000000000	0.166666666666667	0.422222222222222	0.877777777777778	0.450000000000000	0.444444444444444	0	90
0.692307692307693	0.164835164835165	0.428571428571429	0.879120879120879	0.445054945054945	0.450549450549451	0	91
0.701086956521740	0.163043478260870	0.423913043478261	0.869565217391304	0.456521739130435	0.445652173913043	0	92
0.693548387096775	0.161290322580645	0.430107526881720	0.870967741935484	0.451612903225806	0.451612903225806	0	93
0.686170212765958	0.175531914893617	0.425531914893617	0.861702127659574	0.446808510638298	0.446808510638298	0	94
0.694736842105263	0.173684210526316	0.421052631578947	0.863157894736842	0.442105263157895	0.452631578947368	0	95
0.687500000000000	0.171875000000000	0.427083333333333	0.864583333333333	0.447916666666667	0.447916666666667	0	96
0.695876288659794	0.170103092783505	0.422680412371134	0.865979381443299	0.443298969072165	0.453608247422680	0	97
0.688775510204082	0.168367346938776	0.428571428571429	0.867346938775510	0.448979591836735	0.448979591836735	0	98
0.681818181818182	0.181818181818182	0.424242424242424	0.858585858585859	0.444444444444444	0.444444444444444	0	99
0.690000000000000	0.180000000000000	0.420000000000000	0.860000000000000	0.440000000000000	0.450000000000000	0	100
0.683168316831683	0.178217821782178	0.425742574257426	0.861386138613861	0.445544554455446	0.445544554455446	0	101
0.691176470588236	0.176470588235294	0.421568627450980	0.862745098039216	0.441176470588235	0.450980392156863	0	102
0.684466019417476	0.174757281553398	0.427184466019417	0.864077669902913	0.446601941747573	0.446601941747573	0	103
0.692307692307693	0.173076923076923	0.423076923076923	0.865384615384615	0.442307692307692	0.451923076923077	0	104
0.685714285714286	0.185714285714286	0.419047619047619	0.857142857142857	0.438095238095238	0.447619047619048	0	105
0.679245283018868	0.183962264150943	0.424528301886792	0.858490566037736	0.443396226415094	0.443396226415094	0	106
0.686915887850468	0.182242990654206	0.420560747663551	0.859813084112150	0.439252336448598	0.448598130841122	0	107
0.680555555555556	0.180555555555556	0.425925925925926	0.861111111111111	0.444444444444444	0.444444444444444	0	108
0.688073394495413	0.178899082568807	0.422018348623853	0.862385321100918	0.440366972477064	0.449541284403670	0	109
0.681818181818182	0.177272727272727	0.427272727272727	0.863636363636364	0.445454545454545	0.445454545454545	0	110
0.675675675675676	0.189189189189189	0.423423423423423	0.855855855855856	0.441441441441441	0.441441441441441	0	111
0.683035714285715	0.187500000000000	0.419642857142857	0.857142857142857	0.437500000000000	0.446428571428571	0	112
0.676991150442478	0.185840707964602	0.424778761061947	0.858407079646018	0.442477876106195	0.442477876106195	0	113
0.684210526315790	0.184210526315790	0.421052631578947	0.859649122807018	0.438596491228070	0.447368421052632	0	114
0.678260869565218	0.182608695652174	0.426086956521739	0.860869565217391	0.443478260869565	0.443478260869565	0	115
0.685344827586207	0.181034482758621	0.422413793103448	0.853448275862069	0.439655172413793	0.452586206896552	0	116
0.679487179487180	0.179487179487180	0.427350427350427	0.854700854700855	0.444444444444444	0.448717948717949	0	117
0.673728813559322	0.190677966101695	0.423728813559322	0.847457627118644	0.440677966101695	0.444915254237288	0	118
0.680672268907563	0.189075630252101	0.420168067226891	0.848739495798319	0.445378151260504	0.441176470588235	0	119
0.675000000000000	0.187500000000000	0.425000000000000	0.850000000000000	0.441666666666667	0.445833333333333	0	120
0.681818181818182	0.185950413223141	0.421487603305785	0.851239669421488	0.446280991735537	0.442148760330579	0	121
0.676229508196722	0.184426229508197	0.426229508196721	0.852459016393443	0.442622950819672	0.446721311475410	0	122
0.670731707317073	0.195121951219512	0.422764227642276	0.845528455284553	0.439024390243902	0.443089430894309	0	123
0.677419354838710	0.193548387096774	0.419354838709677	0.846774193548387	0.443548387096774	0.439516129032258	0	124
0.672000000000000	0.192000000000000	0.424000000000000	0.848000000000000	0.440000000000000	0.444000000000000	0	125
0.678571428571429	0.190476190476191	0.420634920634921	0.849206349206349	0.444444444444444	0.440476190476190	0	126
0.673228346456693	0.188976377952756	0.425196850393701	0.850393700787402	0.440944881889764	0.444881889763780	0	127
0.679687500000000	0.187500000000000	0.421875000000000	0.851562500000000	0.445312500000000	0.441406250000000	0	128
0.674418604651163	0.197674418604651	0.418604651162791	0.844961240310078	0.441860465116279	0.437984496124031	0	129
0.669230769230769	0.196153846153846	0.423076923076923	0.846153846153846	0.438461538461538	0.442307692307692	0	130
0.675572519083970	0.194656488549618	0.419847328244275	0.847328244274809	0.442748091603053	0.438931297709924	0	131
0.670454545454546	0.193181818181818	0.424242424242424	0.848484848484849	0.439393939393939	0.443181818181818	0	132
0.676691729323309	0.191729323308271	0.421052631578947	0.849624060150376	0.443609022556391	0.439849624060150	0	133
0.671641791044776	0.190298507462687	0.425373134328358	0.850746268656716	0.440298507462687	0.444029850746269	0	134
0.666666666666667	0.200000000000000	0.422222222222222	0.844444444444444	0.437037037037037	0.440740740740741	0	135
0.672794117647059	0.198529411764706	0.419117647058824	0.845588235294118	0.441176470588235	0.437500000000000	0	136
0.667883211678832	0.197080291970803	0.423357664233577	0.846715328467153	0.437956204379562	0.441605839416058	0	137
0.673913043478261	0.195652173913044	0.420289855072464	0.847826086956522	0.442028985507246	0.438405797101449	0	138
0.669064748201439	0.194244604316547	0.424460431654676	0.848920863309353	0.438848920863309	0.442446043165468	0	139
0.675000000000000	0.192857142857143	0.421428571428571	0.842857142857143	0.446428571428571	0.439285714285714	0	140
0.670212765957447	0.191489361702128	0.425531914893617	0.843971631205674	0.443262411347518	0.443262411347518	0	141
0.665492957746479	0.200704225352113	0.422535211267606	0.838028169014085	0.440140845070423	0.440140845070423	0	142
0.671328671328672	0.199300699300699	0.419580419580420	0.839160839160839	0.437062937062937	0.444055944055944	0	143
0.666666666666667	0.197916666666667	0.423611111111111	0.840277777777778	0.440972222222222	0.440972222222222	0	144
0.672413793103449	0.196551724137931	0.420689655172414	0.841379310344828	0.437931034482759	0.444827586206897	0	145
0.667808219178083	0.195205479452055	0.424657534246575	0.842465753424658	0.441780821917808	0.441780821917808	0	146
0.663265306122449	0.204081632653061	0.421768707482993	0.836734693877551	0.438775510204082	0.438775510204082	0	147
0.668918918918919	0.202702702702703	0.418918918918919	0.837837837837838	0.435810810810811	0.442567567567568	0	148
0.664429530201343	0.201342281879195	0.422818791946309	0.838926174496644	0.439597315436242	0.439597315436242	0	149
0.670000000000000	0.200000000000000	0.420000000000000	0.840000000000000	0.436666666666667	0.443333333333333	0	150
0.665562913907285	0.198675496688742	0.423841059602649	0.841059602649007	0.440397350993377	0.440397350993377	0	151
0.671052631578948	0.197368421052632	0.421052631578947	0.842105263157895	0.437500000000000	0.444078947368421	0	152
0.666666666666667	0.205882352941177	0.418300653594771	0.836601307189543	0.434640522875817	0.441176470588235	0	153
0.662337662337663	0.204545454545455	0.422077922077922	0.837662337662338	0.438311688311688	0.438311688311688	0	154
0.667741935483871	0.203225806451613	0.419354838709677	0.838709677419355	0.435483870967742	0.441935483870968	0	155
0.663461538461539	0.201923076923077	0.423076923076923	0.839743589743590	0.439102564102564	0.439102564102564	0	156
0.668789808917198	0.200636942675159	0.420382165605096	0.840764331210191	0.436305732484076	0.442675159235669	0	157
0.664556962025317	0.199367088607595	0.424050632911392	0.841772151898734	0.439873417721519	0.439873417721519	0	158
0.660377358490566	0.207547169811321	0.421383647798742	0.836477987421384	0.437106918238994	0.437106918238994	0	159
0.665625000000001	0.206250000000000	0.418750000000000	0.837500000000000	0.434375000000000	0.440625000000000	0	160
0.661490683229814	0.204968944099379	0.422360248447205	0.838509316770186	0.437888198757764	0.437888198757764	0	161
0.666666666666667	0.203703703703704	0.419753086419753	0.839506172839506	0.435185185185185	0.441358024691358	0	162
0.662576687116565	0.202453987730061	0.423312883435583	0.840490797546012	0.438650306748466	0.438650306748466	0	163
0.667682926829269	0.201219512195122	0.420731707317073	0.835365853658537	0.435975609756098	0.445121951219512	0	164
0.663636363636364	0.200000000000000	0.424242424242424	0.836363636363636	0.439393939393939	0.442424242424242	0	165
0.659638554216868	0.207831325301205	0.421686746987952	0.831325301204819	0.436746987951807	0.439759036144578	0	166
0.664670658682635	0.206586826347305	0.419161676646707	0.832335329341317	0.440119760479042	0.437125748502994	0	167
0.660714285714286	0.205357142857143	0.422619047619048	0.833333333333333	0.437500000000000	0.440476190476190	0	168
0.665680473372782	0.204142011834320	0.420118343195266	0.834319526627219	0.440828402366864	0.437869822485207	0	169
0.661764705882353	0.202941176470588	0.423529411764706	0.835294117647059	0.438235294117647	0.441176470588235	0	170
0.657894736842106	0.210526315789474	0.421052631578947	0.830409356725146	0.435672514619883	0.438596491228070	0	171
0.662790697674419	0.209302325581395	0.418604651162791	0.831395348837209	0.438953488372093	0.436046511627907	0	172
0.658959537572255	0.208092485549133	0.421965317919075	0.832369942196532	0.436416184971098	0.439306358381503	0	173
0.663793103448276	0.206896551724138	0.419540229885057	0.833333333333333	0.439655172413793	0.436781609195402	0	174
0.660000000000000	0.205714285714286	0.422857142857143	0.834285714285714	0.437142857142857	0.440000000000000	0	175
0.656250000000000	0.213068181818182	0.420454545454545	0.829545454545455	0.434659090909091	0.437500000000000	0	176
0.661016949152543	0.211864406779661	0.418079096045198	0.830508474576271	0.437853107344633	0.435028248587571	0	177
0.657303370786517	0.210674157303371	0.421348314606742	0.831460674157303	0.435393258426966	0.438202247191011	0	178
0.662011173184358	0.209497206703911	0.418994413407821	0.832402234636872	0.438547486033520	0.435754189944134	0	179
0.658333333333334	0.208333333333333	0.422222222222222	0.833333333333333	0.436111111111111	0.438888888888889	0	180
0.662983425414365	0.207182320441989	0.419889502762431	0.834254143646409	0.439226519337017	0.436464088397790	0	181
0.659340659340660	0.214285714285714	0.417582417582418	0.829670329670330	0.436813186813187	0.434065934065934	0	182
0.655737704918033	0.213114754098361	0.420765027322404	0.830601092896175	0.434426229508197	0.437158469945355	0	183
0.660326086956522	0.211956521739130	0.418478260869565	0.831521739130435	0.437500000000000	0.434782608695652	0	184
0.656756756756757	0.210810810810811	0.421621621621622	0.832432432432433	0.435135135135135	0.437837837837838	0	185
0.661290322580646	0.209677419354839	0.419354838709677	0.827956989247312	0.440860215053763	0.435483870967742	0	186
0.657754010695188	0.208556149732620	0.422459893048128	0.828877005347594	0.438502673796791	0.438502673796791	0	187
0.662234042553192	0.207446808510638	0.420212765957447	0.829787234042553	0.436170212765957	0.441489361702128	0	188
0.658730158730159	0.214285714285714	0.417989417989418	0.825396825396825	0.433862433862434	0.439153439153439	0	189
0.655263157894737	0.213157894736842	0.421052631578947	0.826315789473684	0.436842105263158	0.436842105263158	0	190
0.659685863874346	0.212041884816754	0.418848167539267	0.827225130890052	0.434554973821990	0.439790575916230	0	191
0.656250000000000	0.210937500000000	0.421875000000000	0.828125000000000	0.437500000000000	0.437500000000000	0	192
0.660621761658031	0.209844559585492	0.419689119170984	0.829015544041451	0.435233160621762	0.440414507772021	0	193
0.657216494845361	0.216494845360825	0.417525773195876	0.824742268041237	0.432989690721650	0.438144329896907	0	194
0.653846153846154	0.215384615384615	0.420512820512821	0.825641025641026	0.435897435897436	0.435897435897436	0	195
0.658163265306123	0.214285714285714	0.418367346938776	0.826530612244898	0.433673469387755	0.438775510204082	0	196
0.654822335025381	0.213197969543147	0.421319796954315	0.827411167512690	0.436548223350254	0.436548223350254	0	197
0.659090909090909	0.212121212121212	0.419191919191919	0.828282828282828	0.434343434343434	0.439393939393939	0	198
0.655778894472362	0.211055276381910	0.422110552763819	0.829145728643216	0.437185929648241	0.437185929648241	0	199
0.652500000000000	0.217500000000000	0.420000000000000	0.825000000000000	0.435000000000000	0.435000000000000	0	200
0.656716417910448	0.216417910447761	0.417910447761194	0.825870646766169	0.432835820895522	0.437810945273632	0	201
0.653465346534654	0.215346534653465	0.420792079207921	0.826732673267327	0.435643564356436	0.435643564356436	0	202
0.657635467980296	0.214285714285714	0.418719211822660	0.827586206896552	0.433497536945813	0.438423645320197	0	203
0.654411764705883	0.213235294117647	0.421568627450980	0.828431372549020	0.436274509803922	0.436274509803922	0	204
0.658536585365854	0.212195121951220	0.419512195121951	0.824390243902439	0.434146341463415	0.441463414634146	0	205
0.655339805825243	0.211165048543689	0.422330097087379	0.825242718446602	0.436893203883495	0.439320388349515	0	206
0.652173913043479	0.217391304347826	0.420289855072464	0.821256038647343	0.434782608695652	0.437198067632850	0	207
0.656250000000000	0.216346153846154	0.418269230769231	0.822115384615385	0.437500000000000	0.435096153846154	0	208
0.653110047846890	0.215311004784689	0.421052631578947	0.822966507177034	0.435406698564593	0.437799043062201	0	209
0.657142857142857	0.214285714285714	0.419047619047619	0.823809523809524	0.438095238095238	0.435714285714286	0	210
0.654028436018958	0.213270142180095	0.421800947867299	0.824644549763033	0.436018957345972	0.438388625592417	0	211
0.650943396226415	0.219339622641509	0.419811320754717	0.820754716981132	0.433962264150943	0.436320754716981	0	212
0.654929577464789	0.218309859154930	0.417840375586854	0.821596244131455	0.436619718309859	0.434272300469484	0	213
0.651869158878505	0.217289719626168	0.420560747663551	0.822429906542056	0.434579439252336	0.436915887850467	0	214
0.655813953488372	0.216279069767442	0.418604651162791	0.823255813953488	0.437209302325581	0.434883720930233	0	215
0.652777777777778	0.215277777777778	0.421296296296296	0.824074074074074	0.435185185185185	0.437500000000000	0	216
0.656682027649770	0.214285714285714	0.419354838709677	0.824884792626728	0.437788018433180	0.435483870967742	0	217
0.653669724770642	0.220183486238532	0.417431192660550	0.821100917431193	0.435779816513761	0.433486238532110	0	218
0.650684931506850	0.219178082191781	0.420091324200913	0.821917808219178	0.433789954337900	0.436073059360731	0	219
0.654545454545455	0.218181818181818	0.418181818181818	0.822727272727273	0.436363636363636	0.434090909090909	0	220
0.651583710407240	0.217194570135747	0.420814479638009	0.823529411764706	0.434389140271493	0.436651583710407	0	221
0.655405405405406	0.216216216216216	0.418918918918919	0.824324324324324	0.436936936936937	0.434684684684685	0	222
0.652466367713005	0.221973094170404	0.417040358744395	0.820627802690583	0.434977578475336	0.432735426008969	0	223
0.649553571428572	0.220982142857143	0.419642857142857	0.821428571428571	0.433035714285714	0.435267857142857	0	224
0.653333333333334	0.220000000000000	0.417777777777778	0.822222222222222	0.435555555555556	0.433333333333333	0	225
0.650442477876106	0.219026548672566	0.420353982300885	0.823008849557522	0.433628318584071	0.435840707964602	0	226
0.654185022026432	0.218061674008811	0.418502202643172	0.823788546255507	0.436123348017621	0.433920704845815	0	227
0.651315789473685	0.217105263157895	0.421052631578947	0.824561403508772	0.434210526315790	0.436403508771930	0	228
0.648471615720524	0.222707423580786	0.419213973799127	0.820960698689956	0.432314410480349	0.434497816593887	0	229
0.652173913043479	0.221739130434783	0.417391304347826	0.821739130434783	0.434782608695652	0.432608695652174	0	230
0.649350649350650	0.220779220779221	0.419913419913420	0.822510822510823	0.432900432900433	0.435064935064935	0	231
0.653017241379311	0.219827586206897	0.418103448275862	0.823275862068966	0.435344827586207	0.433189655172414	0	232
0.650214592274678	0.218884120171674	0.420600858369099	0.824034334763949	0.433476394849785	0.435622317596567	0	233
0.653846153846154	0.217948717948718	0.418803418803419	0.820512820512821	0.438034188034188	0.433760683760684	0	234
0.651063829787234	0.217021276595745	0.421276595744681	0.821276595744681	0.436170212765957	0.436170212765957	0	235
0.648305084745763	0.222457627118644	0.419491525423729	0.817796610169492	0.434322033898305	0.434322033898305	0	236
0.651898734177215	0.221518987341772	0.417721518987342	0.818565400843882	0.432489451476793	0.436708860759494	0	237
0.649159663865547	0.220588235294118	0.420168067226891	0.819327731092437	0.434873949579832	0.434873949579832	0	238
0.652719665271967	0.219665271966527	0.418410041841004	0.820083682008368	0.433054393305439	0.437238493723849	0	239
0.650000000000000	0.218750000000000	0.420833333333333	0.820833333333333	0.435416666666667	0.435416666666667	0	240
0.647302904564316	0.224066390041494	0.419087136929461	0.817427385892116	0.433609958506224	0.433609958506224	0	241
0.650826446280992	0.223140495867769	0.417355371900826	0.818181818181818	0.431818181818182	0.435950413223141	0	242
0.648148148148148	0.222222222222222	0.419753086419753	0.818930041152263	0.434156378600823	0.434156378600823	0	243
0.651639344262295	0.221311475409836	0.418032786885246	0.819672131147541	0.432377049180328	0.436475409836066	0	244
0.648979591836735	0.220408163265306	0.420408163265306	0.820408163265306	0.434693877551020	0.434693877551020	0	245
0.652439024390244	0.219512195121951	0.418699186991870	0.821138211382114	0.432926829268293	0.436991869918699	0	246
0.649797570850203	0.224696356275304	0.417004048582996	0.817813765182186	0.431174089068826	0.435222672064777	0	247
0.647177419354839	0.223790322580645	0.419354838709677	0.818548387096774	0.433467741935484	0.433467741935484	0	248
0.650602409638554	0.222891566265060	0.417670682730924	0.819277108433735	0.431726907630522	0.435742971887550	0	249
0.648000000000000	0.222000000000000	0.420000000000000	0.820000000000000	0.434000000000000	0.434000000000000	0	250
0.651394422310757	0.221115537848606	0.418326693227092	0.820717131474104	0.432270916334661	0.436254980079681	0	251
0.648809523809524	0.220238095238095	0.420634920634921	0.821428571428571	0.434523809523810	0.434523809523810	0	252
0.646245059288538	0.225296442687747	0.418972332015810	0.818181818181818	0.432806324110672	0.432806324110672	0	253
0.649606299212599	0.224409448818898	0.417322834645669	0.818897637795276	0.431102362204724	0.435039370078740	0	254
0.647058823529412	0.223529411764706	0.419607843137255	0.819607843137255	0.433333333333333	0.433333333333333	0	255
0.650390625000000	0.222656250000000	0.417968750000000	0.820312500000000	0.431640625000000	0.435546875000000	0	256
0.647859922178989	0.221789883268482	0.420233463035019	0.821011673151751	0.433852140077821	0.433852140077821	0	257
0.651162790697675	0.220930232558140	0.418604651162791	0.817829457364341	0.432170542635659	0.437984496124031	0	258
0.648648648648649	0.220077220077220	0.420849420849421	0.818532818532819	0.434362934362934	0.436293436293436	0	259
0.646153846153846	0.225000000000000	0.419230769230769	0.815384615384615	0.432692307692308	0.434615384615385	0	260
0.649425287356322	0.224137931034483	0.417624521072797	0.816091954022989	0.434865900383142	0.432950191570881	0	261
0.646946564885496	0.223282442748092	0.419847328244275	0.816793893129771	0.433206106870229	0.435114503816794	0	262
0.650190114068441	0.222433460076046	0.418250950570342	0.817490494296578	0.435361216730038	0.433460076045627	0	263
0.647727272727273	0.221590909090909	0.420454545454545	0.818181818181818	0.433712121212121	0.435606060606061	0	264
0.645283018867925	0.226415094339623	0.418867924528302	0.815094339622642	0.432075471698113	0.433962264150943	0	265
0.648496240601504	0.225563909774436	0.417293233082707	0.815789473684211	0.434210526315790	0.432330827067669	0	266
0.646067415730337	0.224719101123595	0.419475655430712	0.816479400749064	0.432584269662921	0.434456928838951	0	267
0.649253731343284	0.223880597014925	0.417910447761194	0.817164179104478	0.434701492537314	0.432835820895522	0	268
0.646840148698885	0.223048327137546	0.420074349442379	0.817843866171004	0.433085501858736	0.434944237918216	0	269
0.650000000000000	0.222222222222222	0.418518518518519	0.818518518518519	0.435185185185185	0.433333333333333	0	270
0.647601476014760	0.226937269372694	0.416974169741697	0.815498154981550	0.433579335793358	0.431734317343173	0	271
0.645220588235294	0.226102941176471	0.419117647058824	0.816176470588235	0.431985294117647	0.433823529411765	0	272
0.648351648351649	0.225274725274725	0.417582417582418	0.816849816849817	0.434065934065934	0.432234432234432	0	273
0.645985401459854	0.224452554744526	0.419708029197080	0.817518248175182	0.432481751824818	0.434306569343066	0	274
0.649090909090909	0.223636363636364	0.418181818181818	0.818181818181818	0.434545454545455	0.432727272727273	0	275
0.646739130434783	0.228260869565217	0.416666666666667	0.815217391304348	0.432971014492754	0.431159420289855	0	276
0.644404332129964	0.227436823104693	0.418772563176895	0.815884476534296	0.431407942238267	0.433212996389892	0	277
0.647482014388489	0.226618705035971	0.417266187050360	0.816546762589928	0.433453237410072	0.431654676258993	0	278
0.645161290322581	0.225806451612903	0.419354838709677	0.817204301075269	0.431899641577061	0.433691756272401	0	279
0.648214285714286	0.225000000000000	0.417857142857143	0.817857142857143	0.433928571428572	0.432142857142857	0	280
0.645907473309609	0.224199288256228	0.419928825622776	0.818505338078292	0.432384341637011	0.434163701067616	0	281
0.643617021276596	0.228723404255319	0.418439716312057	0.815602836879433	0.430851063829787	0.432624113475177	0	282
0.646643109540636	0.227915194346290	0.416961130742049	0.816254416961131	0.432862190812721	0.431095406360424	0	283
0.644366197183099	0.227112676056338	0.419014084507042	0.816901408450704	0.431338028169014	0.433098591549296	0	284
0.647368421052632	0.226315789473684	0.417543859649123	0.817543859649123	0.433333333333333	0.431578947368421	0	285
0.645104895104895	0.225524475524475	0.419580419580420	0.818181818181818	0.431818181818182	0.433566433566434	0	286
0.648083623693380	0.224738675958188	0.418118466898955	0.815331010452962	0.435540069686411	0.432055749128920	0	287
0.645833333333334	0.223958333333333	0.420138888888889	0.815972222222222	0.434027777777778	0.434027777777778	0	288
0.643598615916955	0.228373702422145	0.418685121107266	0.813148788927336	0.432525951557094	0.432525951557093	0	289
0.646551724137931	0.227586206896552	0.417241379310345	0.813793103448276	0.431034482758621	0.434482758620690	0	290
0.644329896907217	0.226804123711340	0.419243986254296	0.814432989690721	0.432989690721650	0.432989690721649	0	291
0.647260273972603	0.226027397260274	0.417808219178082	0.815068493150685	0.431506849315069	0.434931506849315	0	292
0.645051194539250	0.225255972696246	0.419795221843003	0.815699658703072	0.433447098976109	0.433447098976109	0	293
0.642857142857143	0.229591836734694	0.418367346938776	0.812925170068027	0.431972789115646	0.431972789115646	0	294
0.645762711864407	0.228813559322034	0.416949152542373	0.813559322033898	0.430508474576271	0.433898305084746	0	295
0.643581081081082	0.228040540540541	0.418918918918919	0.814189189189189	0.432432432432432	0.432432432432432	0	296
0.646464646464647	0.227272727272727	0.417508417508418	0.814814814814815	0.430976430976431	0.434343434343434	0	297
0.644295302013423	0.226510067114094	0.419463087248322	0.815436241610738	0.432885906040268	0.432885906040268	0	298
0.647157190635452	0.225752508361204	0.418060200668896	0.816053511705685	0.431438127090301	0.434782608695652	0	299
0.645000000000000	0.230000000000000	0.416666666666667	0.813333333333333	0.430000000000000	0.433333333333333	0	300
0.642857142857143	0.229235880398671	0.418604651162791	0.813953488372093	0.431893687707641	0.431893687707641	0	301
0.645695364238411	0.228476821192053	0.417218543046358	0.814569536423841	0.430463576158940	0.433774834437086	0	302
0.643564356435644	0.227722772277228	0.419141914191419	0.815181518151815	0.432343234323432	0.432343234323432	0	303
0.646381578947369	0.226973684210526	0.417763157894737	0.815789473684210	0.430921052631579	0.434210526315789	0	304
0.644262295081968	0.226229508196721	0.419672131147541	0.816393442622951	0.432786885245902	0.432786885245902	0	305
0.642156862745099	0.230392156862745	0.418300653594771	0.813725490196078	0.431372549019608	0.431372549019608	0	306
0.644951140065147	0.229641693811075	0.416938110749186	0.814332247557003	0.429967426710098	0.433224755700326	0	307
0.642857142857143	0.228896103896104	0.418831168831169	0.814935064935065	0.431818181818182	0.431818181818182	0	308
0.645631067961166	0.228155339805825	0.417475728155340	0.815533980582524	0.430420711974110	0.433656957928802	0	309
0.643548387096775	0.227419354838710	0.419354838709677	0.816129032258064	0.432258064516129	0.432258064516129	0	310
0.646302250803859	0.226688102893891	0.418006430868167	0.813504823151125	0.430868167202572	0.435691318327974	0	311
0.644230769230770	0.225961538461538	0.419871794871795	0.814102564102564	0.432692307692308	0.434294871794872	0	312
0.642172523961662	0.230031948881789	0.418530351437700	0.811501597444089	0.431309904153355	0.432907348242811	0	313
0.644904458598727	0.229299363057325	0.417197452229299	0.812101910828025	0.433121019108280	0.431528662420382	0	314
0.642857142857143	0.228571428571429	0.419047619047619	0.812698412698413	0.431746031746032	0.433333333333333	0	315
0.645569620253165	0.227848101265823	0.417721518987342	0.813291139240506	0.433544303797468	0.431962025316456	0	316
0.643533123028392	0.227129337539432	0.419558359621451	0.813880126182965	0.432176656151420	0.433753943217665	0	317
0.641509433962265	0.231132075471698	0.418238993710692	0.811320754716981	0.430817610062893	0.432389937106918	0	318
0.644200626959248	0.230407523510972	0.416927899686520	0.811912225705329	0.432601880877743	0.431034482758621	0	319
0.642187500000001	0.229687500000000	0.418750000000000	0.812500000000000	0.431250000000000	0.432812500000000	0	320
0.644859813084113	0.228971962616822	0.417445482866044	0.813084112149533	0.433021806853583	0.431464174454829	0	321
0.642857142857143	0.228260869565217	0.419254658385093	0.813664596273292	0.431677018633540	0.433229813664596	0	322
0.645510835913313	0.227554179566563	0.417956656346749	0.814241486068111	0.433436532507740	0.431888544891641	0	323
0.643518518518519	0.231481481481481	0.416666666666667	0.811728395061728	0.432098765432099	0.430555555555555	0	324
0.641538461538462	0.230769230769231	0.418461538461538	0.812307692307692	0.430769230769231	0.432307692307692	0	325
0.644171779141105	0.230061349693251	0.417177914110429	0.812883435582822	0.432515337423313	0.430981595092024	0	326
0.642201834862386	0.229357798165138	0.418960244648318	0.813455657492355	0.431192660550459	0.432721712538226	0	327
0.644817073170732	0.228658536585366	0.417682926829268	0.814024390243902	0.432926829268293	0.431402439024390	0	328
0.642857142857143	0.232522796352584	0.416413373860182	0.811550151975684	0.431610942249240	0.430091185410334	0	329
0.640909090909091	0.231818181818182	0.418181818181818	0.812121212121212	0.430303030303030	0.431818181818182	0	330
0.643504531722055	0.231117824773414	0.416918429003021	0.812688821752266	0.432024169184290	0.430513595166163	0	331
0.641566265060242	0.230421686746988	0.418674698795181	0.813253012048193	0.430722891566265	0.432228915662650	0	332
0.644144144144145	0.229729729729730	0.417417417417417	0.813813813813814	0.432432432432432	0.430930930930931	0	333
0.642215568862276	0.229041916167665	0.419161676646707	0.814371257485030	0.431137724550898	0.432634730538922	0	334
0.640298507462687	0.232835820895522	0.417910447761194	0.811940298507463	0.429850746268657	0.431343283582089	0	335
0.642857142857144	0.232142857142857	0.416666666666667	0.812500000000000	0.431547619047619	0.430059523809524	0	336
0.640949554896143	0.231454005934718	0.418397626112760	0.813056379821958	0.430267062314540	0.431750741839762	0	337
0.643491124260356	0.230769230769231	0.417159763313610	0.813609467455621	0.431952662721894	0.430473372781065	0	338
0.641592920353983	0.230088495575221	0.418879056047198	0.814159292035398	0.430678466076696	0.432153392330383	0	339
0.644117647058824	0.229411764705882	0.417647058823529	0.811764705882353	0.433823529411765	0.430882352941176	0	340
0.642228739002933	0.228739002932551	0.419354838709677	0.812316715542522	0.432551319648094	0.432551319648094	0	341
0.640350877192983	0.232456140350877	0.418128654970760	0.809941520467836	0.431286549707602	0.431286549707602	0	342
0.642857142857144	0.231778425655977	0.416909620991254	0.810495626822158	0.430029154518950	0.432944606413994	0	343
0.640988372093024	0.231104651162791	0.418604651162791	0.811046511627907	0.431686046511628	0.431686046511628	0	344
0.643478260869566	0.230434782608696	0.417391304347826	0.811594202898551	0.430434782608696	0.433333333333333	0	345
0.641618497109827	0.229768786127168	0.419075144508671	0.812138728323699	0.432080924855491	0.432080924855491	0	346
0.639769452449568	0.233429394812680	0.417867435158501	0.809798270893372	0.430835734870317	0.430835734870317	0	347
0.642241379310346	0.232758620689655	0.416666666666667	0.810344827586207	0.429597701149425	0.432471264367816	0	348
0.640401146131806	0.232091690544413	0.418338108882522	0.810888252148997	0.431232091690544	0.431232091690544	0	349
0.642857142857144	0.231428571428571	0.417142857142857	0.811428571428571	0.430000000000000	0.432857142857143	0	350
0.641025641025642	0.230769230769231	0.418803418803419	0.811965811965812	0.431623931623932	0.431623931623932	0	351
0.643465909090910	0.230113636363636	0.417613636363636	0.812500000000000	0.430397727272727	0.433238636363636	0	352
0.641643059490086	0.233711048158640	0.416430594900850	0.810198300283286	0.429178470254958	0.432011331444759	0	353
0.639830508474577	0.233050847457627	0.418079096045198	0.810734463276836	0.430790960451977	0.430790960451977	0	354
0.642253521126761	0.232394366197183	0.416901408450704	0.811267605633803	0.429577464788732	0.432394366197183	0	355
0.640449438202248	0.231741573033708	0.418539325842697	0.811797752808989	0.431179775280899	0.431179775280899	0	356
0.642857142857144	0.231092436974790	0.417366946778712	0.812324929971989	0.429971988795518	0.432773109243697	0	357
0.641061452513967	0.230446927374302	0.418994413407821	0.812849162011173	0.431564245810056	0.431564245810056	0	358
0.639275766016714	0.233983286908078	0.417827298050139	0.810584958217270	0.430362116991643	0.430362116991643	0	359
0.641666666666667	0.233333333333333	0.416666666666667	0.811111111111111	0.429166666666667	0.431944444444444	0	360
0.639889196675901	0.232686980609418	0.418282548476454	0.811634349030471	0.430747922437673	0.430747922437673	0	361
0.642265193370166	0.232044198895028	0.417127071823204	0.812154696132597	0.429558011049724	0.432320441988950	0	362
0.640495867768596	0.231404958677686	0.418732782369146	0.812672176308540	0.431129476584022	0.431129476584022	0	363
0.642857142857144	0.230769230769231	0.417582417582418	0.810439560439560	0.429945054945055	0.434065934065934	0	364
0.641095890410960	0.230136986301370	0.419178082191781	0.810958904109589	0.431506849315069	0.432876712328767	0	365
0.639344262295083	0.233606557377049	0.418032786885246	0.808743169398907	0.430327868852459	0.431693989071038	0	366
0.641689373297003	0.232970027247956	0.416893732970027	0.809264305177112	0.431880108991826	0.430517711171662	0	367
0.639945652173914	0.232336956521739	0.418478260869565	0.809782608695652	0.430706521739130	0.432065217391304	0	368
0.642276422764228	0.231707317073171	0.417344173441734	0.810298102981030	0.432249322493225	0.430894308943089	0	369
0.640540540540541	0.231081081081081	0.418918918918919	0.810810810810811	0.431081081081081	0.432432432432432	0	370
0.638814016172507	0.234501347708895	0.417789757412399	0.808625336927224	0.429919137466307	0.431266846361186	0	371
0.641129032258065	0.233870967741935	0.416666666666667	0.809139784946237	0.431451612903226	0.430107526881720	0	372
0.639410187667561	0.233243967828418	0.418230563002681	0.809651474530831	0.430294906166220	0.431635388739946	0	373
0.641711229946525	0.232620320855615	0.417112299465241	0.810160427807487	0.431818181818182	0.430481283422460	0	374
0.640000000000001	0.232000000000000	0.418666666666667	0.810666666666667	0.430666666666667	0.432000000000000	0	375
0.642287234042554	0.231382978723404	0.417553191489362	0.811170212765958	0.432180851063830	0.430851063829787	0	376
0.640583554376659	0.234748010610080	0.416445623342175	0.809018567639257	0.431034482758621	0.429708222811671	0	377
0.638888888888890	0.234126984126984	0.417989417989418	0.809523809523810	0.429894179894180	0.431216931216931	0	378
0.641160949868075	0.233509234828496	0.416886543535620	0.810026385224274	0.431398416886544	0.430079155672823	0	379
0.639473684210527	0.232894736842105	0.418421052631579	0.810526315789474	0.430263157894737	0.431578947368421	0	380
0.641732283464568	0.232283464566929	0.417322834645669	0.811023622047244	0.431758530183727	0.430446194225722	0	381
0.640052356020943	0.235602094240838	0.416230366492147	0.808900523560210	0.430628272251309	0.429319371727749	0	382
0.638381201044387	0.234986945169713	0.417754569190601	0.809399477806789	0.429503916449086	0.430809399477807	0	383
0.640625000000001	0.234375000000000	0.416666666666667	0.809895833333333	0.430989583333333	0.429687500000000	0	384
0.638961038961040	0.233766233766234	0.418181818181818	0.810389610389610	0.429870129870130	0.431168831168831	0	385
0.641191709844560	0.233160621761658	0.417098445595855	0.810880829015544	0.431347150259067	0.430051813471502	0	386
0.639534883720931	0.232558139534884	0.418604651162791	0.811369509043928	0.430232558139535	0.431524547803617	0	387
0.637886597938145	0.235824742268041	0.417525773195876	0.809278350515464	0.429123711340206	0.430412371134021	0	388
0.640102827763497	0.235218508997429	0.416452442159383	0.809768637532134	0.430591259640103	0.429305912596401	0	389
0.638461538461539	0.234615384615385	0.417948717948718	0.810256410256410	0.429487179487179	0.430769230769231	0	390
0.640664961636829	0.234015345268542	0.416879795396419	0.810741687979540	0.430946291560102	0.429667519181586	0	391
0.639030612244898	0.233418367346939	0.418367346938776	0.811224489795918	0.429846938775510	0.431122448979592	0	392
0.641221374045802	0.232824427480916	0.417302798982188	0.809160305343512	0.432569974554707	0.430025445292621	0	393
0.639593908629442	0.232233502538071	0.418781725888325	0.809644670050762	0.431472081218274	0.431472081218274	0	394
0.637974683544304	0.235443037974684	0.417721518987342	0.807594936708861	0.430379746835443	0.430379746835443	0	395
0.640151515151516	0.234848484848485	0.416666666666667	0.808080808080808	0.429292929292929	0.431818181818182	0	396
0.638539042821159	0.234256926952141	0.418136020151134	0.808564231738035	0.430730478589421	0.430730478589421	0	397
0.640703517587940	0.233668341708543	0.417085427135678	0.809045226130653	0.429648241206030	0.432160804020100	0	398
0.639097744360903	0.233082706766917	0.418546365914787	0.809523809523810	0.431077694235589	0.431077694235589	0	399
0.637500000000001	0.236250000000000	0.417500000000000	0.807500000000000	0.430000000000000	0.430000000000000	0	400
0.639650872817956	0.235660847880299	0.416458852867830	0.807980049875312	0.431421446384040	0	0	401
0.638059701492538	0.235074626865672	0.417910447761194	0.808457711442786	0.432835820895522	0	0	402
0.640198511166254	0.234491315136476	0.416873449131514	0.808933002481390	0.434243176178660	0	0	403
0.638613861386139	0.237623762376238	0.415841584158416	0.806930693069307	0.433168316831683	0	0	404
0.637037037037038	0.237037037037037	0.417283950617284	0.807407407407408	0.434567901234568	0	0	405
0.639162561576355	0.236453201970443	0.416256157635468	0.807881773399015	0.435960591133005	0	0	406
0.637592137592138	0.235872235872236	0.417690417690418	0.808353808353808	0.437346437346437	0	0	407
0.636029411764707	0.238970588235294	0.416666666666667	0.806372549019608	0.436274509803922	0	0	408
0.638141809290954	0.238386308068460	0.415647921760391	0.806845965770171	0.437652811735941	0	0	409
0.636585365853659	0.237804878048780	0.417073170731707	0.807317073170732	0.439024390243902	0	0	410
0.638686131386862	0.237226277372263	0.416058394160584	0.807785888077859	0.440389294403893	0	0	411
0.637135922330098	0.240291262135922	0.415048543689320	0.805825242718447	0.439320388349515	0	0	412
0.635593220338984	0.239709443099274	0.416464891041162	0.806295399515739	0.440677966101695	0	0	413
0.637681159420291	0.239130434782609	0.415458937198068	0.806763285024155	0.442028985507246	0	0	414
0.636144578313254	0.238554216867470	0.416867469879518	0.807228915662651	0.443373493975904	0	0	415
0.634615384615385	0.241586538461538	0.415865384615385	0.805288461538462	0.442307692307692	0	0	416
0.636690647482015	0.241007194244604	0.414868105515588	0.805755395683453	0.443645083932854	0	0	417
0.635167464114833	0.240430622009569	0.416267942583732	0.806220095693780	0.444976076555024	0	0	418
0.637231503579953	0.239856801909308	0.415274463007160	0.806682577565632	0.446300715990453	0	0	419
0.635714285714286	0.242857142857143	0.414285714285714	0.804761904761905	0.445238095238095	0	0	420
0.634204275534443	0.242280285035629	0.415676959619953	0.805225653206651	0.446555819477435	0	0	421
0.636255924170617	0.241706161137441	0.414691943127962	0.805687203791469	0.447867298578199	0	0	422
0.634751773049646	0.241134751773050	0.416075650118203	0.806146572104019	0.449172576832151	0	0	423
0.633254716981133	0.244103773584906	0.415094339622642	0.804245283018868	0.448113207547170	0	0	424
0.635294117647060	0.243529411764706	0.414117647058824	0.804705882352941	0.449411764705882	0	0	425
0.633802816901409	0.242957746478873	0.415492957746479	0.805164319248826	0.450704225352113	0	0	426
0.635831381733022	0.242388758782201	0.414519906323185	0.805620608899297	0.451990632318501	0	0	427
0.634345794392524	0.245327102803738	0.413551401869159	0.803738317757009	0.450934579439252	0	0	428
0.632867132867134	0.244755244755245	0.414918414918415	0.804195804195804	0.452214452214452	0	0	429
0.634883720930233	0.244186046511628	0.413953488372093	0.804651162790698	0.453488372093023	0	0	430
0.633410672853829	0.243619489559165	0.415313225058005	0.805104408352668	0.454756380510441	0	0	431
0.635416666666667	0.243055555555556	0.414351851851852	0.805555555555556	0.456018518518519	0	0	432
0.633949191685913	0.245958429561201	0.413394919168591	0.803695150115473	0.454965357967667	0	0	433
0.632488479262674	0.245391705069124	0.414746543778802	0.804147465437788	0.456221198156682	0	0	434
0.634482758620690	0.244827586206897	0.413793103448276	0.804597701149425	0.457471264367816	0	0	435
0.633027522935781	0.244266055045872	0.415137614678899	0.805045871559633	0.458715596330275	0	0	436
0.633867276887873	0.245995423340961	0.414187643020595	0.803203661327231	0.457665903890160	0	0	437
0.632420091324202	0.245433789954338	0.415525114155251	0.803652968036530	0.458904109589041	0	0	438
0.634396355353076	0.244874715261959	0.414578587699317	0.804100227790433	0.460136674259681	0	0	439
0.632954545454546	0.244318181818182	0.415909090909091	0.804545454545455	0.461363636363636	0	0	440
0.633786848072563	0.246031746031746	0.414965986394558	0.802721088435374	0.460317460317460	0	0	441
0.632352941176471	0.245475113122172	0.416289592760181	0.803167420814480	0.461538461538462	0	0	442
0.634311512415351	0.244920993227991	0.415349887133183	0.803611738148984	0.462753950338600	0	0	443
0.632882882882884	0.247747747747748	0.414414414414414	0.801801801801802	0.461711711711712	0	0	444
0.634831460674158	0.247191011235955	0.413483146067416	0.802247191011236	0.462921348314607	0	0	445
0.633408071748880	0.246636771300448	0.414798206278027	0.802690582959641	0.464125560538117	0	0	446
0.635346756152126	0.246085011185682	0.413870246085011	0.803131991051454	0.465324384787472	0	0	447
0.633928571428572	0.245535714285714	0.415178571428571	0.803571428571429	0.466517857142857	0	0	448
0.632516703786192	0.248329621380846	0.414253897550111	0.801781737193764	0.465478841870824	0	0	449
0.634444444444445	0.247777777777778	0.413333333333333	0.802222222222222	0.466666666666667	0	0	450
0.633037694013305	0.247228381374723	0.414634146341463	0.802660753880266	0.467849223946785	0	0	451
0.634955752212390	0.246681415929204	0.413716814159292	0.803097345132743	0.469026548672566	0	0	452
0.633554083885210	0.249448123620309	0.412803532008830	0.801324503311258	0.467991169977925	0	0	453
0.632158590308371	0.248898678414097	0.414096916299559	0.801762114537445	0.469162995594714	0	0	454
0.634065934065935	0.248351648351648	0.413186813186813	0.802197802197802	0.470329670329670	0	0	455
0.632675438596492	0.247807017543860	0.414473684210526	0.802631578947369	0.471491228070175	0	0	456
0.634573304157550	0.247264770240700	0.413566739606127	0.803063457330416	0.472647702407002	0	0	457
0.633187772925765	0.250000000000000	0.412663755458515	0.801310043668122	0.471615720524017	0	0	458
0.631808278867103	0.249455337690632	0.413943355119826	0.801742919389978	0.472766884531590	0	0	459
0.633695652173914	0.248913043478261	0.413043478260870	0.802173913043478	0.473913043478261	0	0	460
0.632321041214751	0.248373101952278	0.414316702819957	0.802603036876356	0.475054229934924	0	0	461
0.633116883116884	0.250000000000000	0.413419913419913	0.800865800865801	0.474025974025974	0	0	462
0.631749460043197	0.249460043196544	0.414686825053996	0.801295896328294	0.475161987041037	0	0	463
0.633620689655173	0.248922413793103	0.413793103448276	0.801724137931035	0.476293103448276	0	0	464
0.632258064516130	0.248387096774194	0.415053763440860	0.802150537634409	0.477419354838710	0	0	465
0.633047210300430	0.250000000000000	0.414163090128755	0.800429184549356	0.476394849785408	0	0	466
0.631691648822271	0.249464668094218	0.415417558886510	0.800856531049251	0.477516059957173	0	0	467
0.633547008547009	0.248931623931624	0.414529914529915	0.801282051282051	0.478632478632479	0	0	468
0.632196162046909	0.251599147121535	0.413646055437100	0.799573560767591	0.477611940298507	0	0	469
0.634042553191490	0.251063829787234	0.412765957446809	0.800000000000000	0.478723404255319	0	0	470
0.632696390658175	0.250530785562633	0.414012738853503	0.800424628450106	0.479830148619958	0	0	471
0.631355932203391	0.250000000000000	0.415254237288136	0.800847457627119	0.480932203389831	0	0	472
0.633192389006343	0.249471458773784	0.414376321353066	0.801268498942918	0.482029598308668	0	0	473
0.631856540084389	0.252109704641350	0.413502109704641	0.799578059071730	0.481012658227848	0	0	474
0.633684210526316	0.251578947368421	0.412631578947368	0.800000000000000	0.482105263157895	0	0	475
0.632352941176471	0.251050420168067	0.413865546218487	0.800420168067227	0.483193277310924	0	0	476
0.631027253668764	0.250524109014675	0.415094339622642	0.800838574423480	0.484276729559748	0	0	477
0.632845188284519	0.250000000000000	0.414225941422594	0.801255230125523	0.485355648535565	0	0	478
0.631524008350731	0.252609603340292	0.413361169102297	0.799582463465553	0.484342379958246	0	0	479
0.633333333333334	0.252083333333333	0.412500000000000	0.800000000000000	0.485416666666667	0	0	480
0.632016632016633	0.251559251559251	0.413721413721414	0.800415800415800	0.486486486486487	0	0	481
0.633817427385893	0.251037344398340	0.412863070539419	0.800829875518672	0.487551867219917	0	0	482
0.632505175983438	0.250517598343685	0.414078674948240	0.801242236024845	0.488612836438923	0	0	483
0.631198347107439	0.253099173553719	0.413223140495868	0.799586776859504	0.487603305785124	0	0	484
0.632989690721650	0.252577319587629	0.412371134020619	0.800000000000000	0.488659793814433	0	0	485
0.631687242798355	0.252057613168724	0.413580246913580	0.800411522633745	0.489711934156379	0	0	486
0.633470225872691	0.251540041067762	0.412731006160164	0.800821355236140	0.490759753593429	0	0	487
0.632172131147542	0.251024590163934	0.413934426229508	0.801229508196721	0.491803278688525	0	0	488
0.630879345603273	0.253578732106339	0.413087934560327	0.799591002044990	0.490797546012270	0	0	489
0.632653061224490	0.253061224489796	0.412244897959184	0.800000000000000	0.491836734693878	0	0	490
0.631364562118127	0.252545824847250	0.413441955193483	0.800407331975560	0.492871690427699	0	0	491
0.633130081300814	0.252032520325203	0.412601626016260	0.800813008130081	0.493902439024390	0	0	492
0.631845841784991	0.254563894523327	0.411764705882353	0.799188640973631	0.492900608519270	0	0	493
0.630566801619434	0.254048582995951	0.412955465587045	0.799595141700405	0.493927125506073	0	0	494
0.632323232323233	0.253535353535353	0.412121212121212	0.800000000000000	0.494949494949495	0	0	495
0.631048387096775	0.253024193548387	0.413306451612903	0.800403225806452	0.495967741935484	0	0	496
0.632796780684105	0.252515090543260	0.412474849094567	0.800804828973843	0.496981891348089	0	0	497
0.631526104417671	0.255020080321285	0.411646586345382	0.799196787148594	0.495983935742972	0	0	498
0.630260521042085	0.254509018036072	0.412825651302605	0.799599198396794	0.496993987975952	0	0	499
0.632000000000001	0.254000000000000	0.412000000000000	0.800000000000000	0.498000000000000	0	0	500
0.630738522954092	0.253493013972056	0.413173652694611	0.800399201596806	0.499001996007984	0	0	501
0.632470119521913	0.252988047808765	0.412350597609562	0.800796812749004	0.500000000000000	0	0	502
0.631212723658052	0.255467196819085	0.411530815109344	0.799204771371769	0.499005964214712	0	0	503
0.629960317460318	0.254960317460317	0.412698412698413	0.799603174603175	0.500000000000000	0	0	504
0.631683168316832	0.254455445544554	0.411881188118812	0.800000000000000	0.500990099009901	0	0	505
0.630434782608696	0.253952569169960	0.413043478260870	0.800395256916996	0.501976284584980	0	0	506
0.631163708086786	0.255424063116371	0.412228796844181	0.798816568047337	0.500986193293886	0	0	507
0.629921259842520	0.254921259842520	0.413385826771654	0.799212598425197	0.501968503937008	0	0	508
0.631630648330060	0.254420432220039	0.412573673870334	0.799607072691552	0.502946954813360	0	0	509
0.630392156862746	0.253921568627451	0.413725490196078	0.800000000000000	0.503921568627451	0	0	510
0.631115459882584	0.255381604696673	0.412915851272016	0.798434442270059	0.502935420743640	0	0	511
0.629882812500001	0.254882812500000	0.414062500000000	0.798828125000000	0.503906250000000	0	0	512
0.631578947368422	0.254385964912281	0.413255360623782	0.799220272904483	0.504873294346979	0	0	513
0.630350194552530	0.253891050583657	0.414396887159533	0.799610894941634	0.505836575875486	0	0	514
0.629126213592234	0.256310679611650	0.413592233009709	0.798058252427184	0.504854368932039	0	0	515
0.630813953488373	0.255813953488372	0.412790697674419	0.798449612403101	0.505813953488372	0	0	516
0.629593810444875	0.255319148936170	0.413926499032882	0.798839458413927	0.506769825918762	0	0	517
0.631274131274132	0.254826254826255	0.413127413127413	0.799227799227799	0.507722007722008	0	0	518
0.630057803468209	0.257225433526011	0.412331406551060	0.797687861271676	0.506743737957611	0	0	519
0.628846153846154	0.256730769230769	0.413461538461538	0.798076923076923	0.507692307692308	0	0	520
0.630518234165068	0.256238003838771	0.412667946257198	0.798464491362764	0.508637236084453	0	0	521
0.629310344827587	0.255747126436781	0.413793103448276	0.798850574712644	0.509578544061303	0	0	522
0.630975143403442	0.255258126195029	0.413001912045889	0.799235181644360	0.510516252390057	0	0	523
0.629770992366413	0.257633587786259	0.412213740458015	0.797709923664122	0.509541984732824	0	0	524
0.628571428571429	0.257142857142857	0.413333333333333	0.798095238095238	0.510476190476191	0	0	525
0.630228136882130	0.256653992395437	0.412547528517110	0.798479087452472	0.511406844106464	0	0	526
0.629032258064517	0.256166982922201	0.413662239089184	0.798861480075901	0.512333965844402	0	0	527
0.630681818181819	0.255681818181818	0.412878787878788	0.799242424242424	0.513257575757576	0	0	528
0.629489603024575	0.258034026465028	0.412098298676749	0.797731568998110	0.512287334593573	0	0	529
0.628301886792453	0.257547169811321	0.413207547169811	0.798113207547170	0.513207547169811	0	0	530
0.629943502824859	0.257062146892655	0.412429378531073	0.798493408662900	0.514124293785311	0	0	531
0.628759398496241	0.256578947368421	0.413533834586466	0.798872180451128	0.515037593984962	0	0	532
0.629455909943715	0.257973733583490	0.412757973733583	0.797373358348968	0.514071294559099	0	0	533
0.631086142322098	0.257490636704120	0.411985018726592	0.797752808988764	0.514981273408240	0	0	534
0.629906542056075	0.257009345794392	0.413084112149533	0.798130841121495	0.515887850467290	0	0	535
0.628731343283583	0.256529850746269	0.414179104477612	0.798507462686567	0.516791044776119	0	0	536
0.629422718808194	0.257914338919925	0.413407821229050	0.797020484171322	0.515828677839851	0	0	537
0.631040892193309	0.257434944237918	0.412639405204461	0.797397769516729	0.516728624535316	0	0	538
0.629870129870130	0.256957328385900	0.413729128014842	0.797773654916512	0.517625231910946	0	0	539
0.628703703703704	0.259259259259259	0.412962962962963	0.796296296296296	0.516666666666667	0	0	540
0.630314232902034	0.258780036968577	0.412199630314233	0.796672828096118	0.517560073937153	0	0	541
0.629151291512916	0.258302583025830	0.413284132841328	0.797047970479705	0.518450184501845	0	0	542
0.630755064456722	0.257826887661142	0.412523020257827	0.797421731123389	0.519337016574586	0	0	543
0.629595588235295	0.257352941176470	0.413602941176471	0.797794117647059	0.520220588235294	0	0	544
0.628440366972478	0.259633027522936	0.412844036697248	0.796330275229358	0.519266055045872	0	0	545
0.630036630036631	0.259157509157509	0.412087912087912	0.796703296703297	0.520146520146520	0	0	546
0.628884826325412	0.258683729433272	0.413162705667276	0.797074954296161	0.521023765996344	0	0	547
0.630474452554745	0.258211678832117	0.412408759124088	0.797445255474452	0.521897810218978	0	0	548
0.629326047358835	0.257741347905282	0.413479052823315	0.797814207650273	0.522768670309654	0	0	549
0.628181818181819	0.260000000000000	0.412727272727273	0.796363636363636	0.521818181818182	0	0	550
0.629764065335754	0.259528130671506	0.411978221415608	0.796733212341198	0.522686025408348	0	0	551
0.628623188405798	0.259057971014493	0.413043478260870	0.797101449275362	0.523550724637681	0	0	552
0.630198915009042	0.258589511754069	0.412296564195298	0.797468354430380	0.524412296564195	0	0	553
0.629061371841156	0.260830324909747	0.411552346570397	0.796028880866426	0.523465703971119	0	0	554
0.627927927927928	0.260360360360360	0.412612612612613	0.796396396396396	0.524324324324324	0	0	555
0.629496402877698	0.259892086330935	0.411870503597122	0.796762589928058	0.525179856115108	0	0	556
0.628366247755835	0.259425493716337	0.412926391382406	0.797127468581688	0.526032315978456	0	0	557
0.629928315412187	0.258960573476702	0.412186379928315	0.797491039426523	0.526881720430108	0	0	558
0.628801431127013	0.261180679785331	0.411449016100179	0.796064400715563	0.525939177101968	0	0	559
0.627678571428572	0.260714285714286	0.412500000000000	0.796428571428571	0.526785714285714	0	0	560
0.629233511586453	0.260249554367201	0.411764705882353	0.796791443850267	0.527629233511586	0	0	561
0.628113879003559	0.259786476868327	0.412811387900356	0.797153024911032	0.528469750889680	0	0	562
0.629662522202487	0.259325044404973	0.412078152753108	0.797513321492007	0.529307282415631	0	0	563
0.628546099290781	0.261524822695035	0.411347517730496	0.796099290780142	0.528368794326241	0	0	564
0.627433628318585	0.261061946902655	0.412389380530973	0.796460176991150	0.529203539823009	0	0	565
0.628975265017668	0.260600706713781	0.411660777385159	0.796819787985866	0.530035335689046	0	0	566
0.627865961199295	0.260141093474427	0.412698412698413	0.797178130511464	0.530864197530864	0	0	567
0.629401408450705	0.259683098591549	0.411971830985916	0.797535211267605	0.531690140845070	0	0	568
0.628295254833041	0.261862917398945	0.411247803163445	0.796133567662566	0.530755711775044	0	0	569
0.627192982456141	0.261403508771930	0.412280701754386	0.796491228070175	0.531578947368421	0	0	570
0.628721541155867	0.260945709281961	0.411558669001751	0.796847635726795	0.532399299474606	0	0	571
0.627622377622378	0.260489510489510	0.412587412587413	0.797202797202797	0.533216783216783	0	0	572
0.628272251308901	0.261780104712042	0.411867364746946	0.795811518324607	0.532286212914485	0	0	573
0.627177700348433	0.261324041811847	0.412891986062718	0.796167247386759	0.533101045296167	0	0	574
0.628695652173913	0.260869565217391	0.412173913043478	0.796521739130434	0.533913043478261	0	0	575
0.627604166666667	0.260416666666666	0.413194444444444	0.796875000000000	0.534722222222222	0	0	576
0.628249566724437	0.261698440207972	0.412478336221837	0.795493934142114	0.533795493934142	0	0	577
0.627162629757786	0.261245674740484	0.413494809688581	0.795847750865052	0.534602076124567	0	0	578
0.628670120898101	0.260794473229706	0.412780656303972	0.796200345423143	0.535405872193437	0	0	579
0.627586206896552	0.262931034482758	0.412068965517241	0.794827586206896	0.534482758620690	0	0	580
0.629087779690190	0.262478485370052	0.411359724612737	0.795180722891566	0.535283993115318	0	0	581
0.628006872852234	0.262027491408935	0.412371134020619	0.795532646048110	0.536082474226804	0	0	582
0.629502572898800	0.261578044596912	0.411663807890223	0.795883361921097	0.536878216123499	0	0	583
0.628424657534247	0.261130136986301	0.412671232876712	0.796232876712329	0.537671232876712	0	0	584
0.627350427350428	0.263247863247863	0.411965811965812	0.794871794871795	0.536752136752137	0	0	585
0.628839590443686	0.262798634812287	0.411262798634812	0.795221843003413	0.537542662116041	0	0	586
0.627768313458263	0.262350936967632	0.412265758091993	0.795570698466780	0.538330494037479	0	0	587
0.629251700680273	0.261904761904762	0.411564625850340	0.795918367346938	0.539115646258503	0	0	588
0.628183361629882	0.261460101867572	0.412563667232598	0.796264855687606	0.539898132427844	0	0	589
0.627118644067797	0.263559322033898	0.411864406779661	0.794915254237288	0.538983050847457	0	0	590
0.628595600676819	0.263113367174281	0.411167512690355	0.795262267343485	0.539763113367174	0	0	591
0.627533783783784	0.262668918918919	0.412162162162162	0.795608108108108	0.540540540540540	0	0	592
0.629005059021923	0.262225969645868	0.411467116357504	0.795952782462057	0.541315345699831	0	0	593
0.627946127946128	0.261784511784512	0.412457912457912	0.796296296296296	0.542087542087542	0	0	594
0.626890756302521	0.263865546218487	0.411764705882353	0.794957983193277	0.541176470588235	0	0	595
0.628355704697987	0.263422818791946	0.411073825503356	0.795302013422819	0.541946308724832	0	0	596
0.627303182579565	0.262981574539363	0.412060301507538	0.795644891122278	0.542713567839196	0	0	597
0.628762541806021	0.262541806020067	0.411371237458194	0.795986622073578	0.543478260869565	0	0	598
0.627712854757930	0.262103505843072	0.412353923205342	0.796327212020033	0.544240400667779	0	0	599
0.626666666666667	0.264166666666667	0.411666666666667	0.795000000000000	0.543333333333333	0	0	600
0.628119800332779	0.263727121464226	0.410981697171381	0.795341098169717	0.544093178036605	0	0	601
0.627076411960133	0.263289036544851	0.411960132890365	0.795681063122923	0.544850498338870	0	0	602
0.628524046434495	0.262852404643449	0.411276948590381	0.796019900497512	0.545605306799336	0	0	603
0.627483443708610	0.264900662251656	0.410596026490066	0.794701986754967	0.544701986754966	0	0	604
0.626446280991736	0.264462809917355	0.411570247933884	0.795041322314049	0.545454545454545	0	0	605
0.627887788778878	0.264026402640264	0.410891089108911	0.795379537953795	0.546204620462046	0	0	606
0.626853377265240	0.263591433278418	0.411861614497529	0.794069192751235	0.546952224052718	0	0.00164744645799012	607
0.628289473684211	0.263157894736842	0.411184210526316	0.794407894736842	0.547697368421052	0	0.00164473684210526	608
0.627257799671593	0.262725779967159	0.412151067323481	0.793103448275862	0.548440065681445	0	0.00328407224958949	609
0.628688524590164	0.262295081967213	0.411475409836066	0.793442622950820	0.549180327868852	0	0.00327868852459016	610
0.627659574468086	0.261865793780687	0.412438625204583	0.792144026186579	0.549918166939443	0	0.00490998363338789	611
0.626633986928105	0.263888888888889	0.411764705882353	0.790849673202614	0.549019607843137	0	0.00490196078431373	612
0.628058727569332	0.263458401305057	0.411092985318108	0.791190864600326	0.549755301794453	0	0.00489396411092985	613
0.627035830618893	0.263029315960912	0.412052117263844	0.789902280130293	0.550488599348534	0	0.00651465798045603	614
0.628455284552846	0.262601626016260	0.411382113821138	0.790243902439024	0.551219512195121	0	0.00650406504065041	615
0.627435064935065	0.262175324675325	0.412337662337662	0.788961038961039	0.551948051948051	0	0.00811688311688312	616
0.628849270664506	0.261750405186386	0.411669367909238	0.789303079416531	0.552674230145867	0	0.00810372771474878	617
0.627831715210356	0.261326860841424	0.412621359223301	0.788025889967637	0.553398058252427	0	0.00970873786407767	618
0.626817447495962	0.263327948303716	0.411954765751212	0.786752827140549	0.552504038772213	0	0.00969305331179321	619
0.628225806451613	0.262903225806452	0.411290322580645	0.787096774193548	0.553225806451612	0	0.00967741935483871	620
0.627214170692432	0.262479871175523	0.412238325281804	0.785829307568438	0.553945249597423	0	0.0112721417069243	621
0.628617363344052	0.262057877813505	0.411575562700965	0.786173633440514	0.554662379421221	0	0.0112540192926045	622
0.627608346709471	0.261637239165329	0.412520064205457	0.784911717495987	0.555377207062600	0	0.0128410914927769	623
0.629006410256411	0.261217948717949	0.411858974358974	0.785256410256410	0.556089743589743	0	0.0128205128205128	624
0.628000000000000	0.262400000000000	0.411200000000000	0.784000000000000	0.555200000000000	0	0.0144000000000000	625
0.626996805111821	0.261980830670927	0.412140575079872	0.784345047923322	0.555910543130990	0	0.0143769968051118	626
0.628389154704945	0.261562998405104	0.411483253588517	0.784688995215311	0.556618819776714	0	0.0143540669856459	627
0.627388535031848	0.261146496815287	0.412420382165605	0.783439490445860	0.557324840764331	0	0.0159235668789809	628
0.626391096979333	0.262321144674086	0.411764705882353	0.782193958664547	0.556438791732909	0	0.0174880763116057	629
0.627777777777778	0.261904761904762	0.411111111111111	0.782539682539682	0.557142857142857	0	0.0174603174603175	630
0.626782884310619	0.261489698890650	0.412044374009509	0.781299524564184	0.557844690966719	0	0.0190174326465927	631
0.628164556962026	0.261075949367089	0.411392405063291	0.781645569620253	0.558544303797468	0	0.0189873417721519	632
0.627172195892576	0.260663507109005	0.412322274881517	0.780410742496050	0.559241706161137	0	0.0205371248025276	633
0.626182965299685	0.261829652996845	0.411671924290221	0.779179810725552	0.558359621451104	0	0.0220820189274448	634
0.627559055118111	0.261417322834646	0.411023622047244	0.779527559055118	0.559055118110236	0	0.0220472440944882	635
0.626572327044026	0.261006289308176	0.411949685534591	0.779874213836478	0.559748427672956	0	0.0220125786163522	636
0.625588697017269	0.262166405023548	0.411302982731554	0.778649921507064	0.558869701726844	0	0.0235478806907378	637
0.626959247648903	0.261755485893417	0.410658307210031	0.778996865203761	0.559561128526645	0	0.0235109717868339	638
0.625978090766824	0.261345852895149	0.411580594679186	0.777777777777778	0.560250391236306	0	0.0250391236306729	639
0.627343750000000	0.260937500000000	0.410937500000000	0.778125000000000	0.560937500000000	0	0.0250000000000000	640
0.626365054602185	0.260530421216849	0.411856474258970	0.776911076443057	0.561622464898596	0	0.0265210608424337	641
0.627725856697820	0.260124610591900	0.411214953271028	0.777258566978193	0.562305295950155	0	0.0264797507788162	642
0.626749611197512	0.261275272161742	0.410575427682737	0.776049766718507	0.561430793157076	0	0.0279937791601866	643
0.625776397515529	0.260869565217391	0.411490683229814	0.776397515527950	0.562111801242236	0	0.0279503105590062	644
0.627131782945737	0.260465116279070	0.410852713178295	0.776744186046511	0.562790697674418	0	0.0279069767441860	645
0.626160990712075	0.261609907120743	0.410216718266254	0.775541795665635	0.561919504643963	0	0.0294117647058824	646
0.625193199381763	0.261205564142195	0.411128284389490	0.774343122102009	0.562596599690881	0	0.0309119010819165	647
0.626543209876544	0.260802469135803	0.410493827160494	0.774691358024691	0.563271604938271	0	0.0308641975308642	648
0.625577812018491	0.260400616332820	0.411402157164869	0.773497688751926	0.563944530046225	0	0.0323574730354391	649
0.626923076923078	0.260000000000000	0.410769230769231	0.773846153846154	0.564615384615384	0	0.0323076923076923	650
0.625960061443933	0.261136712749616	0.410138248847926	0.772657450076805	0.563748079877112	0	0.0337941628264209	651
0.625000000000001	0.260736196319018	0.411042944785276	0.773006134969325	0.564417177914110	0	0.0337423312883436	652
0.626339969372129	0.260336906584992	0.410413476263400	0.773353751914242	0.565084226646248	0	0.0336906584992343	653
0.625382262996943	0.259938837920489	0.411314984709480	0.772171253822630	0.565749235474006	0	0.0351681957186544	654
0.624427480916031	0.261068702290076	0.410687022900763	0.770992366412214	0.564885496183206	0	0.0366412213740458	655
0.625762195121952	0.260670731707317	0.410060975609756	0.771341463414634	0.565548780487805	0	0.0365853658536585	656
0.624809741248098	0.260273972602740	0.410958904109589	0.770167427701674	0.566210045662100	0	0.0380517503805175	657
0.626139817629180	0.259878419452888	0.410334346504559	0.770516717325228	0.566869300911854	0	0.0379939209726444	658
0.625189681335357	0.261001517450683	0.409711684370258	0.769347496206373	0.566009104704097	0	0.0394537177541730	659
0.624242424242425	0.260606060606061	0.410606060606061	0.769696969696969	0.566666666666666	0	0.0393939393939394	660
0.625567322239032	0.260211800302572	0.409984871406959	0.770045385779122	0.567322239031770	0	0.0393343419062027	661
0.624622356495469	0.259818731117825	0.410876132930514	0.768882175226586	0.567975830815710	0	0.0407854984894260	662
0.623680241327301	0.260935143288085	0.410256410256410	0.767722473604826	0.567119155354449	0	0.0422322775263952	663
0.625000000000001	0.260542168674699	0.409638554216867	0.768072289156626	0.567771084337349	0	0.0421686746987952	664
0.624060150375941	0.260150375939850	0.410526315789474	0.766917293233082	0.568421052631579	0	0.0436090225563910	665
0.625375375375376	0.259759759759760	0.409909909909910	0.767267267267267	0.569069069069069	0	0.0435435435435435	666
0.624437781109446	0.260869565217391	0.409295352323838	0.766116941529235	0.568215892053973	0	0.0449775112443778	667
0.623502994011977	0.260479041916168	0.410179640718563	0.766467065868263	0.568862275449102	0	0.0449101796407186	668
0.624813153961137	0.260089686098655	0.409566517189836	0.766816143497758	0.569506726457399	0	0.0448430493273543	669
0.623880597014926	0.259701492537314	0.410447761194030	0.765671641791044	0.570149253731343	0	0.0462686567164179	670
0.622950819672132	0.260804769001490	0.409836065573771	0.764530551415797	0.569299552906110	0	0.0476900149031297	671
0.624255952380953	0.260416666666667	0.409226190476190	0.764880952380952	0.569940476190476	0	0.0476190476190476	672
0.623328380386331	0.260029717682021	0.410104011887073	0.763744427934621	0.570579494799405	0	0.0490341753343239	673
0.624629080118695	0.259643916913947	0.409495548961424	0.764094955489614	0.571216617210682	0	0.0489614243323442	674
0.623703703703704	0.260740740740741	0.408888888888889	0.762962962962963	0.570370370370370	0	0.0503703703703704	675
0.622781065088758	0.260355029585799	0.409763313609467	0.763313609467455	0.571005917159763	0	0.0502958579881657	676
0.624076809453472	0.259970457902511	0.409158050221566	0.763663220088626	0.571639586410635	0	0.0502215657311669	677
0.623156342182892	0.259587020648968	0.410029498525074	0.762536873156342	0.572271386430678	0	0.0516224188790560	678
0.622238586156113	0.260677466863034	0.409425625920471	0.761413843888070	0.571428571428571	0	0.0530191458026510	679
0.623529411764707	0.260294117647059	0.408823529411765	0.761764705882353	0.572058823529412	0	0.0529411764705882	680
0.622613803230544	0.259911894273128	0.409691629955947	0.760646108663730	0.572687224669603	0	0.0543318649045521	681
0.623900293255133	0.259530791788857	0.409090909090909	0.760997067448680	0.573313782991202	0	0.0542521994134897	682
0.622986822840411	0.260614934114202	0.408491947291362	0.759882869692533	0.572474377745241	0	0.0556368960468521	683
0.622076023391814	0.260233918128655	0.409356725146199	0.760233918128655	0.573099415204678	0	0.0555555555555556	684
0.623357664233577	0.259854014598540	0.408759124087591	0.760583941605839	0.573722627737226	0	0.0554744525547445	685
0.622448979591837	0.259475218658892	0.409620991253644	0.759475218658892	0.574344023323615	0	0.0568513119533528	686
0.621542940320234	0.260553129548763	0.409024745269287	0.758369723435225	0.573508005822416	0	0.0582241630276565	687
0.622819767441861	0.260174418604651	0.408430232558140	0.758720930232558	0.574127906976744	0	0.0581395348837209	688
0.621915820029028	0.259796806966619	0.409288824383164	0.757619738751814	0.574746008708273	0	0.0595065312046444	689
0.623188405797102	0.259420289855073	0.408695652173913	0.757971014492753	0.575362318840579	0	0.0594202898550725	690
0.622286541244574	0.260492040520984	0.408104196816208	0.756874095513748	0.574529667149059	0	0.0607814761215630	691
0.621387283236995	0.260115606936416	0.408959537572254	0.757225433526011	0.575144508670520	0	0.0606936416184971	692
0.622655122655123	0.259740259740260	0.408369408369408	0.757575757575757	0.575757575757576	0	0.0606060606060606	693
0.621757925072047	0.259365994236311	0.409221902017291	0.756484149855908	0.576368876080691	0	0.0619596541786744	694
0.620863309352519	0.260431654676259	0.408633093525180	0.755395683453237	0.575539568345324	0	0.0633093525179856	695
0.622126436781610	0.260057471264368	0.408045977011494	0.755747126436781	0.576149425287356	0	0.0632183908045977	696
0.621233859397418	0.259684361549498	0.408895265423242	0.754662840746054	0.576757532281205	0	0.0645624103299857	697
0.622492836676219	0.259312320916906	0.408309455587393	0.755014326647564	0.577363896848137	0	0.0644699140401146	698
0.621602288984264	0.260371959942776	0.407725321888412	0.753934191702432	0.576537911301860	0	0.0658082975679542	699
0.620714285714286	0.260000000000000	0.408571428571429	0.754285714285714	0.577142857142857	0	0.0657142857142857	700
0.621968616262483	0.259629101283880	0.407988587731812	0.754636233951498	0.577746077032810	0	0.0656205420827390	701
0.621082621082622	0.259259259259259	0.408831908831909	0.753561253561253	0.578347578347578	0	0.0669515669515670	702
0.620199146514937	0.260312944523471	0.408250355618777	0.752489331436700	0.577524893314367	0	0.0682788051209104	703
0.621448863636364	0.259943181818182	0.407670454545455	0.752840909090909	0.578125000000000	0	0.0681818181818182	704
0.620567375886525	0.259574468085107	0.408510638297872	0.751773049645390	0.578723404255319	0	0.0695035460992908	705
0.621813031161474	0.259206798866856	0.407932011331445	0.752124645892351	0.579320113314448	0	0.0694050991501417	706
0.620933521923622	0.260254596888260	0.407355021216407	0.751060820367751	0.578500707213578	0	0.0707213578500707	707
0.620056497175142	0.259887005649718	0.408192090395480	0.751412429378531	0.579096045197740	0	0.0706214689265537	708
0.621297602256700	0.259520451339915	0.407616361071932	0.751763046544429	0.579689703808180	0	0.0705218617771509	709
0.620422535211268	0.259154929577465	0.408450704225352	0.750704225352112	0.580281690140845	0	0.0718309859154930	710
0.619549929676513	0.260196905766526	0.407876230661041	0.749648382559775	0.579465541490858	0	0.0731364275668073	711
0.620786516853933	0.259831460674157	0.407303370786517	0.750000000000000	0.580056179775281	0	0.0730337078651686	712
0.619915848527350	0.259467040673212	0.408134642356241	0.748948106591865	0.580645161290323	0	0.0743338008415147	713
0.621148459383754	0.259103641456583	0.407563025210084	0.749299719887955	0.581232492997199	0	0.0742296918767507	714
0.620279720279721	0.260139860139860	0.406993006993007	0.748251748251748	0.580419580419580	0	0.0755244755244755	715
0.619413407821230	0.259776536312849	0.407821229050279	0.748603351955307	0.581005586592179	0	0.0754189944134078	716
0.620641562064157	0.259414225941423	0.407252440725244	0.748953974895397	0.581589958158996	0	0.0753138075313808	717
0.619777158774374	0.259052924791086	0.408077994428969	0.747910863509749	0.582172701949861	0	0.0766016713091922	718
0.618915159944368	0.260083449235049	0.407510431154381	0.746870653685674	0.581363004172462	0	0.0778859527121002	719
0.620138888888890	0.259722222222222	0.406944444444444	0.747222222222222	0.581944444444444	0	0.0777777777777778	720
0.619278779472955	0.259361997226075	0.407766990291262	0.746185852981969	0.582524271844660	0	0.0790568654646325	721
0.620498614958449	0.259002770083103	0.407202216066482	0.746537396121883	0.583102493074792	0	0.0789473684210527	722
0.619640387275243	0.260027662517289	0.406639004149378	0.745504840940525	0.582295988934993	0	0.0802213001383126	723
0.618784530386741	0.259668508287293	0.407458563535912	0.745856353591160	0.582872928176795	0	0.0801104972375691	724
0.620000000000001	0.259310344827586	0.406896551724138	0.746206896551724	0.583448275862069	0	0.0800000000000000	725
0.619146005509642	0.258953168044077	0.407713498622590	0.745179063360881	0.584022038567493	0	0.0812672176308540	726
0.618294360385145	0.259972489683631	0.407152682255846	0.744154057771664	0.583218707015131	0	0.0825309491059147	727
0.619505494505495	0.259615384615385	0.406593406593407	0.744505494505494	0.583791208791209	0	0.0824175824175824	728
0.618655692729767	0.259259259259259	0.407407407407407	0.743484224965706	0.584362139917695	0	0.0836762688614541	729
0.619863013698631	0.258904109589041	0.406849315068493	0.743835616438356	0.584931506849315	0	0.0835616438356165	730
0.619015047879618	0.259917920656635	0.406292749658003	0.742818057455540	0.584131326949384	0	0.0848153214774282	731
0.618169398907104	0.259562841530055	0.407103825136612	0.743169398907104	0.584699453551912	0	0.0846994535519126	732
0.619372442019100	0.259208731241474	0.406548431105048	0.743519781718963	0.585266030013642	0	0.0845839017735335	733
0.618528610354224	0.258855585831063	0.407356948228883	0.742506811989101	0.585831062670300	0	0.0858310626702998	734
0.617687074829933	0.259863945578231	0.406802721088435	0.741496598639456	0.585034013605442	0	0.0870748299319728	735
0.618885869565218	0.259510869565218	0.406250000000000	0.741847826086956	0.585597826086956	0	0.0869565217391305	736
0.618046132971507	0.259158751696065	0.407055630936228	0.740841248303935	0.586160108548168	0	0.0881953867028494	737
0.619241192411925	0.258807588075881	0.406504065040650	0.741192411924119	0.586720867208672	0	0.0880758807588076	738
0.618403247631936	0.259810554803789	0.405953991880920	0.740189445196211	0.585926928281461	0	0.0893098782138025	739
0.617567567567568	0.259459459459460	0.406756756756757	0.740540540540540	0.586486486486486	0	0.0891891891891892	740
0.618758434547909	0.259109311740891	0.406207827260459	0.740890688259109	0.587044534412955	0	0.0890688259109312	741
0.617924528301887	0.258760107816712	0.407008086253369	0.739892183288409	0.587601078167116	0	0.0902964959568734	742
0.617092866756394	0.259757738896366	0.406460296096904	0.738896366083445	0.586810228802153	0	0.0915208613728130	743
0.618279569892474	0.259408602150538	0.405913978494624	0.739247311827957	0.587365591397849	0	0.0913978494623656	744
0.617449664429531	0.259060402684564	0.406711409395973	0.738255033557047	0.587919463087248	0	0.0926174496644296	745
0.618632707774800	0.258713136729223	0.406166219839142	0.738605898123324	0.588471849865952	0	0.0924932975871314	746
0.617804551539492	0.259705488621152	0.405622489959839	0.737617135207496	0.587684069611780	0	0.0937081659973227	747
0.616978609625669	0.259358288770054	0.406417112299465	0.737967914438502	0.588235294117647	0	0.0935828877005348	748
0.618157543391189	0.259012016021362	0.405874499332443	0.738317757009346	0.588785046728972	0	0.0934579439252337	749
0.617333333333334	0.258666666666667	0.406666666666667	0.737333333333333	0.589333333333333	0	0.0946666666666667	750
0.616511318242344	0.259653794940080	0.406125166444740	0.736351531291611	0.588548601864181	0	0.0958721704394142	751
0.617686170212767	0.259308510638298	0.405585106382979	0.736702127659574	0.589095744680851	0	0.0957446808510639	752
0.616865869853918	0.258964143426295	0.406374501992032	0.735723771580345	0.589641434262948	0	0.0969455511288181	753
0.618037135278515	0.258620689655173	0.405835543766578	0.736074270557029	0.590185676392573	0	0.0968169761273210	754
0.617218543046358	0.259602649006623	0.405298013245033	0.735099337748344	0.589403973509934	0	0.0980132450331126	755
0.616402116402117	0.259259259259259	0.406084656084656	0.735449735449735	0.589947089947090	0	0.0978835978835979	756
0.617569352708059	0.258916776750330	0.405548216644650	0.735799207397622	0.590488771466314	0	0.0977542932628798	757
0.616754617414249	0.258575197889182	0.406332453825858	0.734828496042216	0.591029023746702	0	0.0989445910290238	758
0.615942028985508	0.259552042160738	0.405797101449275	0.733860342555994	0.590250329380764	0	0.100131752305665	759
0.617105263157896	0.259210526315790	0.405263157894737	0.734210526315789	0.590789473684210	0	0.100000000000000	760
0.616294349540080	0.258869908015769	0.406044678055191	0.733245729303548	0.591327201051248	0	0.101182654402103	761
0.617454068241471	0.258530183727034	0.405511811023622	0.733595800524934	0.591863517060367	0	0.101049868766404	762
0.616644823066842	0.259501965923984	0.404980340760157	0.732634338138925	0.591087811271297	0	0.102228047182176	763
0.615837696335079	0.259162303664922	0.405759162303665	0.732984293193717	0.591623036649215	0	0.102094240837696	764
0.616993464052288	0.258823529411765	0.405228758169935	0.733333333333333	0.592156862745098	0	0.101960784313726	765
0.616187989556137	0.258485639686684	0.406005221932115	0.732375979112271	0.592689295039165	0	0.103133159268930	766
0.615384615384616	0.259452411994785	0.405475880052151	0.731421121251629	0.591916558018253	0	0.104302477183833	767
0.616536458333334	0.259114583333333	0.404947916666667	0.731770833333333	0.592447916666667	0	0.104166666666667	768
0.615734720416126	0.258777633289987	0.405721716514955	0.730819245773732	0.592977893368010	0	0.105331599479844	769
0.616883116883118	0.258441558441559	0.405194805194805	0.731168831168831	0.593506493506494	0	0.105194805194805	770
0.616083009079119	0.259403372243839	0.404669260700389	0.730220492866407	0.592736705577173	0	0.106355382619974	771
0.615284974093265	0.259067357512953	0.405440414507772	0.730569948186528	0.593264248704663	0	0.106217616580311	772
0.616429495472187	0.258732212160414	0.404915912031048	0.730918499353169	0.593790426908150	0	0.106080206985770	773
0.615633074935401	0.258397932816538	0.405684754521964	0.729974160206718	0.594315245478036	0	0.107235142118863	774
0.614838709677420	0.259354838709678	0.405161290322581	0.729032258064516	0.593548387096774	0	0.108387096774194	775
0.615979381443300	0.259020618556701	0.404639175257732	0.729381443298969	0.594072164948454	0	0.108247422680412	776
0.615186615186616	0.258687258687259	0.405405405405405	0.728442728442728	0.594594594594594	0	0.109395109395109	777
0.616323907455014	0.258354755784062	0.404884318766067	0.728791773778920	0.595115681233933	0	0.109254498714653	778
0.615532734274712	0.259306803594352	0.404364569961489	0.727856225930680	0.594351732991014	0	0.110397946084724	779
0.614743589743591	0.258974358974359	0.405128205128205	0.728205128205128	0.594871794871795	0	0.110256410256410	780
0.615877080665814	0.258642765685019	0.404609475032010	0.728553137003841	0.595390524967990	0	0.110115236875800	781
0.615089514066497	0.258312020460358	0.405370843989770	0.727621483375959	0.595907928388747	0	0.111253196930946	782
0.614303959131546	0.259259259259259	0.404853128991060	0.726692209450830	0.595146871008940	0	0.112388250319285	783
0.615433673469389	0.258928571428572	0.404336734693878	0.727040816326530	0.595663265306122	0	0.112244897959184	784
0.614649681528663	0.258598726114650	0.405095541401274	0.726114649681528	0.596178343949045	0	0.113375796178344	785
0.615776081424937	0.258269720101781	0.404580152671756	0.726463104325700	0.596692111959288	0	0.113231552162850	786
0.614993646759848	0.259212198221093	0.404066073697586	0.725540025412960	0.595933926302414	0	0.114358322744600	787
0.614213197969544	0.258883248730965	0.404822335025381	0.725888324873096	0.596446700507614	0	0.114213197969543	788
0.615335868187580	0.258555133079848	0.404309252217997	0.726235741444867	0.596958174904943	0	0.114068441064639	789
0.614556962025317	0.258227848101266	0.405063291139241	0.725316455696202	0.597468354430380	0	0.115189873417722	790
0.613780025284451	0.259165613147914	0.404551201011378	0.724399494310999	0.596713021491782	0	0.116308470290771	791
0.614898989898991	0.258838383838384	0.404040404040404	0.724747474747475	0.597222222222222	0	0.116161616161616	792
0.614123581336697	0.258511979823455	0.404791929382093	0.723833543505674	0.597730138713745	0	0.117276166456494	793
0.615239294710328	0.258186397984887	0.404282115869018	0.724181360201511	0.598236775818640	0	0.117128463476071	794
0.614465408805032	0.259119496855346	0.403773584905660	0.723270440251572	0.597484276729560	0	0.118238993710692	795
0.613693467336684	0.258793969849246	0.404522613065327	0.723618090452261	0.597989949748744	0	0.118090452261307	796
0.614805520702636	0.258469259723965	0.404015056461731	0.723964868255960	0.598494353826851	0	0.117942283563363	797
0.614035087719299	0.258145363408522	0.404761904761905	0.723057644110275	0.598997493734336	0	0.119047619047619	798
0.613266583229037	0.259073842302879	0.404255319148936	0.722152690863579	0.598247809762203	0	0.120150187734668	799
0.614375000000001	0.258750000000000	0.403750000000000	0.722500000000000	0.598750000000000	0	0.120000000000000	800
0.613607990012485	0.258426966292135	0.404494382022472	0.721598002496879	0.599250936329588	0	0.121098626716604	801
0.614713216957607	0.258104738154614	0.403990024937656	0.721945137157107	0.599750623441396	0	0.120947630922693	802
0.613947696139478	0.259028642590287	0.403486924034869	0.721046077210460	0.599003735990037	0	0.122042341220423	803
0.613184079601991	0.258706467661692	0.404228855721393	0.721393034825870	0.599502487562189	0	0.121890547263682	804
0.614285714285715	0.258385093167702	0.403726708074534	0.721739130434782	0.600000000000000	0	0.121739130434783	805
0.613523573200994	0.258064516129033	0.404466501240695	0.720843672456575	0.600496277915632	0	0.122828784119107	806
0.612763320941761	0.259603469640645	0.403965303593556	0.719950433705080	0.599752168525402	0	0.122676579925651	807
0.613861386138615	0.259282178217822	0.403465346534654	0.720297029702970	0.600247524752475	0	0.122524752475248	808
0.613102595797282	0.258961681087763	0.404202719406675	0.719406674907293	0.600741656365884	0	0.123609394313968	809
0.614197530864199	0.258641975308642	0.403703703703704	0.719753086419753	0.601234567901234	0	0.123456790123457	810
0.613440197287301	0.259556103575833	0.403205918618989	0.718865598027127	0.600493218249075	0	0.124537607891492	811
0.612684729064041	0.259236453201971	0.403940886699507	0.717980295566502	0.600985221674877	0	0.125615763546798	812
0.613776137761379	0.258917589175892	0.403444034440344	0.718327183271832	0.601476014760147	0	0.125461254612546	813
0.613022113022114	0.258599508599509	0.404176904176904	0.717444717444717	0.601965601965602	0	0.126535626535627	814
0.614110429447854	0.258282208588957	0.403680981595092	0.717791411042945	0.602453987730061	0	0.126380368098160	815
0.613357843137256	0.259191176470589	0.403186274509804	0.716911764705882	0.601715686274510	0	0.127450980392157	816
0.612607099143208	0.258873929008568	0.403916768665851	0.717258261933904	0.602203182374541	0	0.127294981640147	817
0.613691931540344	0.258557457212714	0.403422982885086	0.717603911980440	0.602689486552567	0	0.127139364303179	818
0.612942612942614	0.259462759462760	0.402930402930403	0.716727716727716	0.601953601953602	0	0.128205128205128	819
0.612195121951221	0.259146341463415	0.403658536585366	0.715853658536585	0.602439024390244	0	0.129268292682927	820
0.613276492082827	0.258830694275274	0.403166869671133	0.716199756394640	0.602923264311815	0	0.129110840438490	821
0.612530413625305	0.258515815085158	0.403892944038929	0.715328467153284	0.603406326034063	0	0.130170316301703	822
0.613608748481168	0.258201701093560	0.403402187120292	0.715674362089915	0.603888213851762	0	0.130012150668287	823
0.612864077669904	0.259101941747573	0.402912621359223	0.714805825242718	0.603155339805825	0	0.131067961165049	824
0.612121212121213	0.258787878787879	0.403636363636364	0.715151515151515	0.603636363636363	0	0.130909090909091	825
0.613196125907992	0.258474576271187	0.403147699757869	0.715496368038741	0.604116222760290	0	0.130750605326877	826
0.612454655380896	0.259371221281742	0.402660217654172	0.714631197097944	0.603385731559855	0	0.131801692865780	827
0.611714975845412	0.259057971014493	0.403381642512077	0.713768115942029	0.603864734299517	0	0.132850241545894	828
0.612786489746684	0.258745476477684	0.402895054282268	0.714113389626055	0.604342581423401	0	0.132689987937274	829
0.612048192771086	0.258433734939759	0.403614457831325	0.713253012048193	0.604819277108433	0	0.133734939759036	830
0.613116726835140	0.258122743682311	0.403128760529483	0.713598074608905	0.605294825511432	0	0.133574007220217	831
0.612379807692309	0.259014423076923	0.402644230769231	0.712740384615384	0.604567307692307	0	0.134615384615385	832
0.611644657863147	0.258703481392557	0.403361344537815	0.713085234093637	0.605042016806722	0	0.134453781512605	833
0.612709832134294	0.258393285371703	0.402877697841727	0.713429256594724	0.605515587529976	0	0.134292565947242	834
0.611976047904193	0.259281437125749	0.402395209580838	0.712574850299401	0.604790419161676	0	0.135329341317365	835
0.611244019138757	0.258971291866029	0.403110047846890	0.711722488038277	0.605263157894737	0	0.136363636363636	836
0.612305854241339	0.258661887694146	0.402628434886499	0.712066905615292	0.605734767025089	0	0.136200716845878	837
0.611575178997615	0.258353221957041	0.403341288782816	0.711217183770883	0.606205250596658	0	0.137231503579952	838
0.612634088200240	0.258045292014303	0.402860548271752	0.711561382598331	0.606674612634088	0	0.137067938021454	839
0.611904761904763	0.258928571428572	0.402380952380952	0.710714285714285	0.605952380952381	0	0.138095238095238	840
0.611177170035673	0.258620689655173	0.403091557669441	0.711058263971462	0.606420927467301	0	0.137931034482759	841
0.612232779097389	0.258313539192399	0.402612826603325	0.711401425178147	0.606888361045130	0	0.137767220902613	842
0.611506524317914	0.259193357058126	0.402135231316726	0.710557532621589	0.606168446026097	0	0.138790035587189	843
0.610781990521328	0.258886255924171	0.402843601895735	0.709715639810426	0.606635071090047	0	0.139810426540284	844
0.611834319526629	0.258579881656805	0.402366863905325	0.710059171597633	0.607100591715976	0	0.139644970414201	845
0.611111111111113	0.258274231678487	0.403073286052010	0.709219858156028	0.607565011820331	0	0.140661938534279	846
0.612160566706023	0.257969303423849	0.402597402597403	0.709563164108618	0.608028335301062	0	0.140495867768595	847
0.611438679245284	0.258844339622642	0.402122641509434	0.708726415094339	0.607311320754717	0	0.141509433962264	848
0.610718492343935	0.258539458186102	0.402826855123675	0.709069493521790	0.607773851590106	0	0.141342756183746	849
0.611764705882354	0.258235294117647	0.402352941176471	0.709411764705882	0.608235294117647	0	0.141176470588235	850
0.611045828437134	0.259106933019977	0.401880141010576	0.708578143360752	0.607520564042303	0	0.142185663924794	851
0.610328638497654	0.258802816901409	0.402582159624413	0.707746478873239	0.607981220657277	0	0.143192488262911	852
0.611371629542792	0.258499413833529	0.402110199296600	0.708089097303634	0.608440797186401	0	0.143024618991794	853
0.610655737704919	0.258196721311476	0.402810304449649	0.707259953161592	0.608899297423887	0	0.144028103044497	854
0.611695906432750	0.257894736842105	0.402339181286550	0.707602339181286	0.609356725146199	0	0.143859649122807	855
0.610981308411216	0.258761682242991	0.401869158878505	0.706775700934579	0.608644859813084	0	0.144859813084112	856
0.610268378063012	0.258459743290549	0.402567094515753	0.707117852975496	0.609101516919486	0	0.144690781796966	857
0.611305361305363	0.258158508158508	0.402097902097902	0.707459207459207	0.609557109557109	0	0.144522144522145	858
0.610593713620490	0.259022118742724	0.401629802095460	0.706635622817229	0.608847497089639	0	0.145518044237486	859
0.609883720930234	0.258720930232558	0.402325581395349	0.705813953488372	0.609302325581395	0	0.146511627906977	860
0.610917537746807	0.258420441347271	0.401858304297329	0.706155632984901	0.609756097560975	0	0.146341463414634	861
0.610208816705338	0.258120649651972	0.402552204176334	0.705336426914153	0.610208816705336	0	0.147331786542924	862
0.611239860950175	0.257821552723059	0.402085747392816	0.705677867902665	0.610660486674391	0	0.147161066048668	863
0.610532407407409	0.258680555555556	0.401620370370370	0.704861111111111	0.609953703703703	0	0.148148148148148	864
0.609826589595377	0.258381502890174	0.402312138728324	0.705202312138728	0.610404624277456	0	0.147976878612717	865
0.610854503464205	0.258083140877598	0.401847575057737	0.705542725173210	0.610854503464203	0	0.147806004618938	866
0.610149942329874	0.258938869665513	0.401384083044983	0.704728950403691	0.610149942329873	0	0.148788927335640	867
0.609447004608296	0.258640552995392	0.402073732718894	0.703917050691244	0.610599078341014	0	0.149769585253456	868
0.610471806674340	0.258342922899885	0.401611047180667	0.704257767548907	0.611047180667434	0	0.149597238204833	869
0.609770114942530	0.258045977011494	0.402298850574713	0.703448275862069	0.611494252873563	0	0.150574712643678	870
0.610792192881747	0.257749712973594	0.401836969001148	0.703788748564868	0.611940298507463	0	0.150401836969001	871
0.610091743119267	0.258600917431193	0.401376146788991	0.702981651376147	0.611238532110092	0	0.151376146788991	872
0.609392898052693	0.258304696449026	0.402061855670103	0.703321878579610	0.611683848797251	0	0.151202749140894	873
0.610411899313503	0.258009153318078	0.401601830663616	0.703661327231121	0.612128146453089	0	0.151029748283753	874
0.609714285714287	0.258857142857143	0.401142857142857	0.702857142857143	0.611428571428571	0	0.152000000000000	875
0.609018264840184	0.258561643835617	0.401826484018265	0.702054794520548	0.611872146118721	0	0.152968036529680	876
0.610034207525657	0.258266818700114	0.401368301026226	0.702394526795895	0.612314709236032	0	0.152793614595211	877
0.609339407744876	0.257972665148064	0.402050113895216	0.701594533029613	0.612756264236902	0	0.153758542141230	878
0.610352673492607	0.257679180887372	0.401592718998862	0.701934015927190	0.613196814562002	0	0.153583617747440	879
0.609659090909092	0.258522727272727	0.401136363636364	0.701136363636363	0.612500000000000	0	0.154545454545455	880
0.608967082860387	0.258229284903519	0.401816118047673	0.701475595913734	0.612939841089671	0	0.154370034052213	881
0.609977324263040	0.257936507936508	0.401360544217687	0.701814058956916	0.613378684807256	0	0.154195011337869	882
0.609286523216309	0.258776896942243	0.400906002265006	0.701019252548131	0.612684031710079	0	0.155152887882220	883
0.608597285067875	0.258484162895928	0.401583710407240	0.700226244343891	0.613122171945701	0	0.156108597285068	884
0.609604519774013	0.258192090395480	0.401129943502825	0.700564971751412	0.613559322033898	0	0.155932203389831	885
0.608916478555306	0.257900677200903	0.401805869074492	0.699774266365688	0.613995485327314	0	0.156884875846501	886
0.609921082299889	0.257609921082300	0.401352874859076	0.700112739571589	0.614430665163472	0	0.156708004509583	887
0.609234234234236	0.259009009009009	0.400900900900901	0.699324324324324	0.613738738738739	0	0.156531531531532	888
0.608548931383578	0.258717660292464	0.401574803149606	0.698537682789651	0.614173228346457	0	0.157480314960630	889
0.609550561797754	0.258426966292135	0.401123595505618	0.698876404494382	0.614606741573033	0	0.157303370786517	890
0.608866442199777	0.258136924803592	0.401795735129068	0.698092031425365	0.615039281705948	0	0.158249158249158	891
0.609865470852019	0.257847533632287	0.401345291479821	0.698430493273542	0.615470852017937	0	0.158071748878924	892
0.609182530795074	0.258678611422172	0.400895856662934	0.697648376259798	0.614781634938410	0	0.159014557670773	893
0.608501118568234	0.258389261744966	0.401565995525727	0.697986577181208	0.615212527964206	0	0.158836689038031	894
0.609497206703912	0.258100558659218	0.401117318435754	0.698324022346369	0.615642458100558	0	0.158659217877095	895
0.608816964285716	0.258928571428571	0.400669642857143	0.697544642857143	0.614955357142857	0	0.159598214285714	896
0.608138238573022	0.258639910813824	0.401337792642141	0.696767001114827	0.615384615384615	0	0.160535117056856	897
0.609131403118041	0.258351893095768	0.400890868596882	0.697104677060133	0.615812917594655	0	0.160356347438753	898
0.608453837597332	0.258064516129032	0.401557285873192	0.696329254727475	0.616240266963292	0	0.161290322580645	899
0.609444444444446	0.257777777777778	0.401111111111111	0.696666666666666	0.616666666666666	0	0.161111111111111	900
0.608768035516095	0.258601553829079	0.400665926748058	0.695893451720311	0.615982241953385	0	0.162042175360710	901
0.608093126385811	0.258314855875832	0.401330376940133	0.696230598669623	0.616407982261641	0	0.161862527716186	902
0.609080841638983	0.258028792912514	0.400885935769657	0.696566998892580	0.616832779623477	0	0.161683277962348	903
0.608407079646019	0.258849557522124	0.400442477876106	0.695796460176991	0.616150442477876	0	0.162610619469027	904
0.607734806629836	0.258563535911602	0.401104972375691	0.695027624309392	0.616574585635359	0	0.163535911602210	905
0.608719646799118	0.258278145695364	0.400662251655629	0.695364238410596	0.616997792494481	0	0.163355408388521	906
0.608048511576628	0.257993384785006	0.401323042998898	0.694597574421168	0.617420066152150	0	0.164277839029769	907
0.609030837004407	0.257709251101322	0.400881057268723	0.694933920704846	0.617841409691630	0	0.164096916299560	908
0.608360836083610	0.258525852585259	0.400440044004400	0.694169416941694	0.617161716171617	0	0.165016501650165	909
0.607692307692309	0.258241758241758	0.401098901098901	0.694505494505494	0.617582417582417	0	0.164835164835165	910
0.608671789242592	0.257958287596048	0.400658616904501	0.694840834248079	0.618002195389681	0	0.164654226125137	911
0.608004385964914	0.258771929824561	0.400219298245614	0.694078947368421	0.617324561403509	0	0.165570175438597	912
0.607338444687844	0.258488499452355	0.400876232201533	0.693318729463308	0.617743702081051	0	0.166484118291347	913
0.608315098468273	0.258205689277899	0.400437636761488	0.693654266958424	0.618161925601750	0	0.166301969365427	914
0.607650273224045	0.257923497267760	0.401092896174863	0.692896174863388	0.618579234972677	0	0.167213114754098	915
0.608624454148473	0.257641921397380	0.400655021834061	0.693231441048035	0.618995633187773	0	0.167030567685590	916
0.607960741548529	0.258451472191930	0.400218102508179	0.692475463467830	0.618320610687023	0	0.167938931297710	917
0.607298474945535	0.258169934640523	0.400871459694989	0.692810457516340	0.618736383442266	0	0.167755991285403	918
0.608269858541895	0.257889009793254	0.400435255712731	0.693144722524483	0.619151251360174	0	0.167573449401523	919
0.607608695652175	0.258695652173913	0.400000000000000	0.692391304347826	0.618478260869565	0	0.168478260869565	920
0.606948968512488	0.258414766558089	0.400651465798046	0.691639522258415	0.618892508143322	0	0.169381107491857	921
0.607917570498917	0.258134490238612	0.400216919739696	0.691973969631236	0.619305856832972	0	0.169197396963124	922
0.607258938244855	0.257854821235103	0.400866738894908	0.691224268689057	0.619718309859155	0	0.170097508125677	923
0.608225108225109	0.257575757575758	0.400432900432900	0.691558441558441	0.620129870129870	0	0.169913419913420	924
0.607567567567569	0.258378378378378	0.400000000000000	0.690810810810811	0.619459459459459	0	0.170810810810811	925
0.606911447084235	0.258099352051836	0.400647948164147	0.691144708423326	0.619870410367170	0	0.170626349892009	926
0.607874865156420	0.257820927723840	0.400215749730313	0.691477885652643	0.620280474649406	0	0.170442286947141	927
0.607219827586208	0.258620689655173	0.399784482758621	0.690732758620689	0.619612068965517	0	0.171336206896552	928
0.606566200215287	0.258342303552207	0.400430570505920	0.689989235737352	0.620021528525296	0	0.172228202368138	929
0.607526881720431	0.258064516129032	0.400000000000000	0.690322580645161	0.620430107526881	0	0.172043010752688	930
0.606874328678841	0.257787325456498	0.400644468313641	0.689581095596133	0.620837808807733	0	0.172932330827068	931
0.607832618025752	0.257510729613734	0.400214592274678	0.689914163090129	0.621244635193133	0	0.172746781115880	932
0.607181136120044	0.258306538049303	0.399785637727760	0.689174705251875	0.620578778135048	0	0.173633440514470	933
0.606531049250537	0.258029978586724	0.400428265524625	0.689507494646681	0.620985010706638	0	0.173447537473233	934
0.607486631016044	0.257754010695187	0.400000000000000	0.689839572192513	0.621390374331551	0	0.173262032085562	935
0.606837606837608	0.258547008547009	0.399572649572650	0.689102564102564	0.620726495726496	0	0.174145299145299	936
0.606189967982926	0.258271077908218	0.400213447171825	0.688367129135539	0.621131270010672	0	0.175026680896478	937
0.607142857142858	0.257995735607676	0.399786780383795	0.688699360341151	0.621535181236674	0	0.174840085287847	938
0.606496272630459	0.257720979765708	0.400425985090522	0.687965921192758	0.621938232161874	0	0.175718849840256	939
0.607446808510640	0.257446808510638	0.400000000000000	0.688297872340425	0.622340425531915	0	0.175531914893617	940
0.606801275239109	0.258235919234857	0.399574920297556	0.687566418703507	0.621679064824654	0	0.176408076514347	941
0.606157112526541	0.257961783439491	0.400212314225053	0.687898089171974	0.622080679405520	0	0.176220806794055	942
0.607104984093320	0.257688229056204	0.399787910922588	0.688229056203605	0.622481442205726	0	0.176033934252386	943
0.606461864406781	0.258474576271187	0.399364406779661	0.687500000000000	0.621822033898305	0	0.176906779661017	944
0.605820105820107	0.258201058201058	0.400000000000000	0.686772486772487	0.622222222222222	0	0.177777777777778	945
0.606765327695562	0.257928118393235	0.399577167019027	0.687103594080338	0.622621564482029	0	0.177589852008457	946
0.606124604012673	0.257655755015840	0.400211193241816	0.686378035902851	0.623020063357972	0	0.178458289334741	947
0.607067510548524	0.257383966244726	0.399789029535865	0.686708860759493	0.623417721518987	0	0.178270042194093	948
0.606427818756587	0.258166491043203	0.399367755532139	0.685985247629083	0.622760800842992	0	0.179135932560590	949
0.605789473684212	0.257894736842105	0.400000000000000	0.686315789473684	0.623157894736842	0	0.178947368421053	950
0.606729758149318	0.257623554153523	0.399579390115668	0.686645636172450	0.623554153522608	0	0.178759200841220	951
0.606092436974791	0.258403361344538	0.399159663865546	0.685924369747899	0.622899159663865	0	0.179621848739496	952
0.605456453305353	0.258132214060861	0.399790136411333	0.685204616998950	0.623294858342077	0	0.180482686253935	953
0.606394129979037	0.257861635220126	0.399371069182390	0.685534591194968	0.623689727463312	0	0.180293501048218	954
0.605759162303666	0.257591623036649	0.400000000000000	0.684816753926701	0.624083769633508	0	0.181151832460733	955
0.606694560669457	0.257322175732218	0.399581589958159	0.685146443514644	0.624476987447699	0	0.180962343096234	956
0.606060606060607	0.258098223615465	0.399164054336468	0.684430512016719	0.623824451410658	0	0.181818181818182	957
0.605427974947809	0.257828810020877	0.399791231732777	0.684759916492693	0.624217118997912	0	0.181628392484342	958
0.606360792492181	0.257559958289885	0.399374348279458	0.685088633993743	0.624608967674661	0	0.181438998957247	959
0.605729166666668	0.258333333333333	0.398958333333333	0.684375000000000	0.623958333333333	0	0.182291666666667	960
0.605098855359002	0.258064516129032	0.399583766909469	0.683662851196670	0.624349635796046	0	0.183142559833507	961
0.606029106029107	0.257796257796258	0.399168399168399	0.683991683991684	0.624740124740125	0	0.182952182952183	962
0.605399792315681	0.257528556593977	0.399792315680166	0.683281412253375	0.625129802699896	0	0.183800623052960	963
0.606327800829877	0.257261410788382	0.399377593360996	0.683609958506224	0.625518672199170	0	0.183609958506224	964
0.605699481865286	0.258549222797928	0.398963730569948	0.682901554404145	0.624870466321243	0	0.183419689119171	965
0.605072463768117	0.258281573498965	0.399585921325052	0.682194616977225	0.625258799171843	0	0.184265010351967	966
0.605997931747674	0.258014477766288	0.399172699069286	0.682523267838676	0.625646328852120	0	0.184074457083764	967
0.605371900826447	0.257747933884298	0.399793388429752	0.681818181818182	0.626033057851239	0	0.184917355371901	968
0.606295149638804	0.257481940144479	0.399380804953560	0.682146542827657	0.626418988648091	0	0.184726522187823	969
0.605670103092785	0.258247422680413	0.398969072164949	0.681443298969072	0.625773195876288	0	0.185567010309278	970
0.605046343975284	0.257981462409887	0.399588053553038	0.681771369721936	0.626158599382080	0	0.185375901132853	971
0.605967078189302	0.257716049382716	0.399176954732510	0.682098765432099	0.626543209876543	0	0.185185185185185	972
0.605344295991779	0.258478931140802	0.398766700924974	0.681397738951696	0.625899280575539	0	0.186022610483042	973
0.604722792607804	0.258213552361396	0.399383983572895	0.680698151950719	0.626283367556468	0	0.186858316221766	974
0.605641025641027	0.257948717948718	0.398974358974359	0.681025641025641	0.626666666666667	0	0.186666666666667	975
0.605020491803280	0.257684426229508	0.399590163934426	0.680327868852459	0.627049180327869	0	0.187500000000000	976
0.605936540429889	0.257420675537359	0.399181166837257	0.680655066530194	0.627430910951893	0	0.187308085977482	977
0.605316973415134	0.258179959100205	0.398773006134969	0.679959100204499	0.626789366053170	0	0.188139059304704	978
0.604698672114404	0.257916241062309	0.399387129724208	0.680286006128703	0.627170582226762	0	0.187946884576098	979
0.605612244897960	0.257653061224490	0.398979591836735	0.680612244897959	0.627551020408163	0	0.187755102040816	980
0.604994903160042	0.258409785932722	0.398572884811417	0.679918450560652	0.626911314984709	0	0.188583078491335	981
0.604378818737272	0.258146639511202	0.399185336048880	0.679226069246436	0.627291242362525	0	0.189409368635438	982
0.605289928789421	0.257884028484232	0.398779247202442	0.679552390640895	0.627670396744659	0	0.189216683621567	983
0.604674796747969	0.257621951219512	0.399390243902439	0.678861788617886	0.628048780487805	0	0.190040650406504	984
0.605583756345179	0.257360406091371	0.398984771573604	0.679187817258883	0.628426395939086	0	0.189847715736041	985
0.604969574036512	0.258113590263692	0.398580121703854	0.678498985801217	0.627789046653144	0	0.190669371196755	986
0.604356636271531	0.257852077001013	0.399189463019250	0.678824721377913	0.628166160081053	0	0.190476190476191	987
0.605263157894738	0.257591093117409	0.398785425101215	0.679149797570850	0.628542510121457	0	0.190283400809717	988
0.604651162790699	0.258341759352882	0.398382204246714	0.678463094034378	0.627906976744186	0	0.191102123356926	989
0.604040404040405	0.258080808080808	0.398989898989899	0.677777777777778	0.628282828282828	0	0.191919191919192	990
0.604944500504542	0.257820383451059	0.398587285570131	0.678102926337033	0.628657921291624	0	0.191725529767911	991
0.604334677419356	0.257560483870968	0.399193548387097	0.677419354838709	0.629032258064516	0	0.192540322580645	992
0.605236656596174	0.257301107754280	0.398791540785499	0.677744209466264	0.629405840886203	0	0.192346424974824	993
0.604627766599599	0.258048289738430	0.398390342052314	0.677062374245473	0.628772635814889	0	0.193158953722334	994
0.604020100502514	0.257788944723618	0.398994974874372	0.677386934673367	0.629145728643216	0	0.192964824120603	995
0.604919678714861	0.257530120481928	0.398594377510040	0.677710843373494	0.629518072289156	0	0.192771084337349	996
0.604312938816451	0.258274824473420	0.398194583751254	0.677031093279839	0.628886659979940	0	0.193580742226680	997
0.603707414829661	0.258016032064128	0.398797595190381	0.676352705410821	0.629258517034068	0	0.194388777555110	998
0.604604604604606	0.257757757757758	0.398398398398398	0.676676676676676	0.629629629629629	0	0.194194194194194	999
0.604000000000001	0.257500000000000	0.399000000000000	0.676000000000000	0.630000000000000	0	0.195000000000000	1000
